Orthogonal decomposition of anisotropic constitutive models for the phase field approach to fracture

We propose a decomposition of constitutive relations into crack-driving and persistent portions, specifically designed for materials with anisotropic/orthotropic behavior in the phase field approach to fracture to account for the tension-compression asymmetry. This decomposition follows a variational framework, satisfying the orthogonality condition for anisotropic materials. This implies that the present model can be applied to arbitrary anisotropic elastic behavior in a three-dimensional setting. On this basis, we generalize two existing models for tension-compression asymmetry in isotropic materials, namely the volumetric-deviatoric model and the no-tension model, towards materials with anisotropic nature. Two benchmark problems, single notched tensile shear tests, are used to study the performance of the present model. The results can retain the anisotropic constitutive behavior and the tension-compression asymmetry in the crack response, and are qualitatively in accordance with the expected behavior for orthotropic materials. Furthermore, to study the direction of maximum energy dissipation, we modify the surface integral based energy release computation, $G_\theta$, to account only for the crack-driving energy. The computed energies with our proposed modifications predict the fracture propagation direction correctly compared with the standard G-theta method.

==> Crack Propagation in Orthotropic Materials/auxil.tex <==
\subsubsection{Tension-compression asymmetry}
%Let $\mathcal{K}$ be the set of all symmetrized second-order tensors, and let $\mathcal{K}^t\in\mathcal{K}$ be a convex subset and $\mathcal{K}^c$ be a polar cone such that $\mathcal{K}^c = \{\bm{e}^c \, \big| \, \bm{e}^c \cdot \bm{e}^t \le 0 \quad  \forall\bm{e}^c \in \mathcal{K}^c \}$.
To account for tension-compression asymmetry, several existing approaches split the sound elastic energy density $\varPsi(\bm{\varepsilon})$ into a crack-driving portion $\varPsi^t(\bm{\varepsilon})$ and a persistent portion $\varPsi^c(\bm{\varepsilon})$. The elastic energy density in \eqref{Eq:pi} is then replaced by the expression
\begin{equation}\label{Eq:psi_deg}
    \begin{aligned}
        \varPsi = g(d)\varPsi^t + \varPsi^c,
    \end{aligned}
\end{equation}
where the damage degradation function $g(d)$ acts only on the crack-driving portion $\varPsi^t$.
We let the partition of the sound elastic energy density be based on that of the strain tensor \[\bm{\varepsilon} = \bm{\varepsilon}^t + \bm{\varepsilon}^c,\] that is, the constitutive behaviors
\begin{equation}\label{Eq:psi_split}
    \begin{aligned}
        \varPsi^t(\bm{\varepsilon}^t) = \frac12 \mathbb{C} \bm{\varepsilon}^t\cdot\bm{\varepsilon}^t, \quad \bm{\sigma}^t = \mathbb{C}\bm{\varepsilon}^t,\\
        \varPsi^c(\bm{\varepsilon}^t) = \frac12 \mathbb{C} \bm{\varepsilon}^c\cdot\bm{\varepsilon}^c, \quad \bm{\sigma}^c = \mathbb{C}\bm{\varepsilon}^c,
    \end{aligned}
\end{equation}
are characterized by the same elasticity tensor $\mathbb{C}$.
% An essential ingredient for developing phase field models resides in the additive decomposition of the strain tensor $\boldsymbol{\varepsilon}$ into a crack-driving portion $\bm{\varepsilon}^t$ and a persistent portion $\bm{\varepsilon}^{c}$ as below,
% \begin{equation}\label{Eq:eps_split}
%     \begin{aligned}
%         \bm{\varepsilon}=\bm{\varepsilon}^{t} + \bm{\varepsilon}^{c}.
%     \end{aligned}
% \end{equation}
% Following \citep{Freddi2010, li2016numerical}, we let the partition of the strain energy density $\varPsi(\bm{\varepsilon})$ be based on that of the strain tensor as in \eqref{Eq:eps_split} such that
\KYtodoi{We should mention other split methods available and emphasize that not all of them meet the orthogonality condition and why it is important to honor the orthogonality condition.}
% \begin{equation}\label{Eq:strain_eng_decomp}
%     \begin{aligned}
%         \varPsi(\bm{\varepsilon}) = \varPsi^t(\bm{\varepsilon}^t) + \varPsi^c(\bm{\varepsilon}^c).
%     \end{aligned}
% \end{equation}
%{For $\bm{\varepsilon}^t\in\mathcal{S}^t$ to be variationally consistent, we have:}
This way, $\bm{\varepsilon}^{t}\in\mathcal{K}^t$ can be determined based on the following variational requirement \citep{Freddi2010, li2016numerical}:
\begin{equation}\label{Eq:loc_variational}
    \begin{aligned}
        \bm{\varepsilon}^t = \underset{\bm{e}^t\in\mathcal{K}^t}{\mrm{argmin}} \, 
        \mathbb{C}\bigl(\bm{\varepsilon} - \bm{e}^t\bigr)\cdot\bigl(\bm{\varepsilon} - \bm{e}^t\bigr),
    \end{aligned}
\end{equation}
where $\mathcal{K}^t$ is a convex subset of the symmetrized second-order tensor. 
From convex analysis, the following inequality should be satisfied:
% Letting $f(\bm{e}^t):= \mathbb{C}(\bm{\varepsilon} - \bm{e}^t)\cdot(\bm{\varepsilon} - \bm{e}^t)$, the following inequality should be satisfied:
\begin{equation}\label{Eq:eps_min}
    \begin{aligned}
        -\mathbb{C}(\bm{\varepsilon} - \bm{\varepsilon}^t)\cdot\bigl(\bm{e}^t - \bm{\varepsilon}^t\bigr) \geq 0,
        % f(\bm{\varepsilon}^t) 
        % &\leq
        % f(\bm{\varepsilon}^t) + \nabla f(\bm{\varepsilon}^t)\cdot(\bm{\varepsilon}^t - \bm{e}^t) 
        % \quad \forall \bm{e}^t\in\mathcal{S}^t.
        % \nabla f(\bm{\varepsilon}^t)\cdot\bigl(\bm{\varepsilon}^t - \bm{e}^t\bigr) \geq 0,
        \quad \forall \bm{e}^t\in\mathcal{K}^t.
    \end{aligned}
\end{equation}
% or equivalently,
% \begin{equation}\label{Eq:eps_min}
%     \begin{aligned}
%         % \mathbb{C}(\bm{\varepsilon} - \bm{\varepsilon}^t)\cdot(\boldsymbol{\eps} - \boldsymbol{\eps}_+) 
%         % &\le
%         %  \mathbb{C}\dcdot(\boldsymbol{\eps} - \boldsymbol{\eps}_+)\dcdot(\boldsymbol{\eps} - \boldsymbol{\eps}_+)
%         % + 2 \mathbb{C}\dcdot(\boldsymbol{\eps} - \boldsymbol{\eps}_+)\dcdot(\boldsymbol{\eps}_+ - \bf{e}_+)
%         \mathbb{C}(\bm{\varepsilon} - \bm{\varepsilon}^t)\cdot(\bm{\varepsilon}^t - \bm{e}^t)\geq 0,
%         \quad \forall \bm{e}^t\in\mathcal{S}^t.
%     \end{aligned}
% \end{equation}
% Thus we have:
% \begin{equation}\label{Eq:eps_inequality}
%     \begin{aligned}
%         0\le \mathbb{C}\dcdot(\boldsymbol{\eps} - \boldsymbol{\eps}_+)\dcdot(\boldsymbol{\eps}_+ - \bf{e}_+).
%     \end{aligned}
% \end{equation}
Testing \eqref{Eq:eps_min} with $\bm{e}^t=2\bm{\varepsilon}^t$ and $\bm{e}^t=\frac{1}{2} \bm{\varepsilon}^t$ yields 
% \[ 0 \leq \mathbb{C} (\bm{\varepsilon}^c\cdot\bm{\varepsilon}^t) \quad \text{and} \quad 0 \leq - \mathbb{C} 
%     (\bm{\varepsilon}^c\cdot\bm{\varepsilon}^t).\]
%\[ \mathbb{C} (\bm{\varepsilon} - \bm{\varepsilon}^t)\cdot\bm{\varepsilon}^t \geq 0 \quad \text{and} \quad - \mathbb{C}  
%(\bm{\varepsilon} - \bm{\varepsilon}^t)\cdot\bm{\varepsilon}^t \geq 0.\]%
the following orthogonality condition:
\begin{equation}\label{Eq:orthogonality}
    \begin{aligned}
        % \mathbb{C}\dcdot\boldsymbol{\varepsilon}_{-}\dcdot\boldsymbol{\eps}_{+}=\mathbb{C}\dcdot\boldsymbol{\varepsilon}_+\dcdot\boldsymbol{\varepsilon}_{-}=0,
        \mathbb{C}\bm{\varepsilon}^t\cdot\bm{\varepsilon}^c = 0.
    \end{aligned}
\end{equation}
% Therefore, the strain energy of a linearly elastic material without damage 
% \[\varPsi(\boldsymbol{\varepsilon}) = \frac12\boldsymbol{\varepsilon}\dcdot\mathbb{C}\dcdot\boldsymbol{\varepsilon}\] 
% is partitioned into two parts which depend on $\bm{\varepsilon}^{t}$ and $\bm{\varepsilon}^{c}$ respectively:
% \begin{equation}\label{Eq:psi_split}
%     \begin{aligned}
%         \varPsi(\boldsymbol{\varepsilon}) = \varPsi^{t}(\boldsymbol{\varepsilon}_+)+\varPsi^{c}(\boldsymbol{\varepsilon}_{-})=\frac12\boldsymbol{\varepsilon}_+\dcdot\mathbb{C}\dcdot\boldsymbol{\varepsilon}_+ + \frac12\boldsymbol{\varepsilon}_-\dcdot\mathbb{C}\dcdot\boldsymbol{\varepsilon}_-.
%     \end{aligned}
% \end{equation}
% Therefore, the necessary and sufficient condition for \eqref{Eq:psi_split} to hold is the orthogonality condition \eqref{Eq:orthogonality}.
This implies that $\varPsi^t$ and $\varPsi^c$ defined in \eqref{Eq:psi_split} constitute indeed a partition of $\varPsi$
\begin{equation*}\label{Eq:psi_halb}
    \begin{aligned}
        2\varPsi = \mathbb{C}\bm{\varepsilon}\cdot\bm{\varepsilon} = \bm{\sigma}^t\cdot\bm{\varepsilon}^t + \bm{\sigma}^c\cdot\bm{\varepsilon}^c,
    \end{aligned}
\end{equation*}
where the crossed terms disappear thanks to the orthogonality condition \eqref{Eq:orthogonality}. \newline
Using this variational formulation in \eqref{Eq:loc_variational}, the tension-compression asymmetry reduces to setting the convex cone $\mathcal{K}^t$ which represents the strain that contributes to damage. \newline
In the sequel, we name two alternatives that we use in this paper.
\paragraph{volumetric-deviatoric}
\paragraph{masonry-like model}
% With the assumption that only the part $\varPsi_{0}(\boldsymbol{\varepsilon}_+)$ contributes to damage, the bulk strain energy of the material with damage takes the form:
% \begin{equation*}
%     \begin{aligned}
%         \varPsi^{\prime}(\boldsymbol{\varepsilon}) = g(d)\varPsi^{t}(\boldsymbol{\varepsilon}_+) + \varPsi^{c}({\boldsymbol{\varepsilon}_-}).
%     \end{aligned}
% \end{equation*}
% \TNtodoi{The degradation function is used here. Later, we should clearly distinguish between $\varPsi$ and $\varPsi_0$ as well as $\boldsymbol\sigma$ and $\boldsymbol\sigma _0$, etc. in the following derivations.}
% \VZRtodoi{Now, I changed $\varPsi_0$ to $\varPsi$ and the degraded $\varPsi$ to $\varPsi^{\prime}$, also introduced $\varPsi^t$ and $\varPsi^c$. I think it's better we first present our split, and the degradation function appears at very end of the stage.}
% %Let $\boldsymbol{\sigma}$ denote the Cauchy stress tensor.
\subsection{General approach to orthogonal decomposition}
\subsubsection*{Governing equations}
We aim at finding $(\bm{\varepsilon}^{t},\bm{\varepsilon}^{c})$ and correspondingly $(\bm{\sigma}^{t}, \bm{\sigma}^{c})$ such that the following set of equations holds:
\begin{subequations}\label{Eq:governing}
    \begin{align}
        \bm{\varepsilon} = \bm{\varepsilon}^{t} + \bm{\varepsilon}^{c}&, \\
        \mathbb{C}\bigl(\bm{\varepsilon}^{t}\cdot\bm{\varepsilon}^{c}\bigr) = 0&, \\
        \bm{\sigma} = \bm{\sigma}^{t} + \bm{\sigma}^{c}&, \\
        \mathbb{S}\bigl(\bm{\sigma}^{t}\cdot\bm{\sigma}^{c}\bigr) = 0&,
        %\boldsymbol{\sigma}^{t}\cdot(\mathbb{C}^{-1}\bm{\sigma}_{-})=0,
    \end{align}
\end{subequations}
where $\mathbb{S}=\mathbb{C}^{-1}$ denotes the compliance tensor, and \[\bm{\sigma}=\mathbb{C}\bm{\varepsilon}.\]
This way, we can partition $\varPsi(\bm{\varepsilon})$ as in \eqref{Eq:psi_split}.

==> Crack Propagation in Orthotropic Materials/conclusion.tex <==
In this paper, we have proposed a method to account for orthotropy/anisotropy of materials when modeling tension-compression asymmetry in their crack response. Two decomposition models, {volumetric-deviatoric} and {no-tension}, were extended to capture arbitrary types of anisotropy in the constitutive behavior in a three-dimensional setting. 
A major characteristic of the formulation is that it keeps the variational formalism in partitioning the constitutive model, honoring the orthogonality condition. \newline
The two models presented in this work were evaluated and compared numerically in a square plate with a pre-notched crack loaded in tension and shear. 
Under the tensile loading, the result indicates that both models have approximately similar responses. Testing different material orientation angles, the effect of orthotropy on the material response is clearly observed. To better interpret the results, we investigated the energy release rate using the $G_\theta$ method with our proposed modifications.
And a significant difference in the resulting crack paths iss observed between the two models under shear loading. However, at this point it is difficult to judge which model provides a more reliable outcome. \newline
The results presented herein highlight the importance of how to decompose the constitutive model of materials with anisotropic nature in the phase field approach to brittle fracture. 
% Comparing the numerical results with experimental tests will be a topic of future study for a better conclusion on the model predictions. 
%\KYtodoi{I don't like this last sentence. It sounds too generic and does not add anything really. I suggest the following as a future study and we can mention comparisons to experiments if you like.}
As opposed to imposing anisotropic behaviors to the surface energy (fracture toughness), adapting the strain energy leads to `weak' anisotropy~\cite{Li2019aniso}.
However, some materials evidently exhibit anisotropic elastic deformation and this effect should not be ignored.
Future studies should include `strong' anisotropy by adding the directionality to the surface energy, and comparisons against experiments to determine whether both strong and weak anisotropy or how much of each is required.


==> Crack Propagation in Orthotropic Materials/formulations.tex <==
This section introduces the theory and implementation details to account for the tension-compression asymmetry in the crack response of anisotropic materials. In \ref{Sec:problem-PF} we recapitulate the basic ingredients of a phase field formulation. Then, in \ref{Sec:problem-transformation} we perform an elastic energy preserving transformation so that an orthogonal decomposition of the strain tensor, and its consequent partitioning of the strain energy density, can be realized in the transformed space. Thereafter, in \ref{Sec:problem-unilateral} we pick the two existing models for the tension-compression asymmetry, {volumetric-deviatoric} and {no-tension}, and adapt them for anisotropic materials. Finally, in \ref{Sec:problem-anisotropy} we provide various types of the elasticity tensors that can be adapted into the model. Readers interested in directly using the model can jump to \eqref{Eq:D_tensors}, \eqref{Eq:strain_decomp_voldev}, \eqref{Eq:sigma}, \eqref{Eq:C_decomp} for anisotropic {volumetric-deviatoric} and \eqref{Eq:proj-dir-dev}, \eqref{Eq:strain_decomp_masonry}, \eqref{Eq:sigma_masonry_tensor}, \eqref{Eq:C_masonry_tensor} for anisotropic {no-tension}.
\subsection{Phase field formulation}\label{Sec:problem-PF}
The phase field formulation for brittle fracture is essentially based on minimization of the following functional
\begin{equation}\label{Eq:pi}
    \begin{aligned}
        \Pi_{\ell}(\boldsymbol{u},d) := \int_{\Omega} \varPsi\bigl[\boldsymbol{\varepsilon}(\boldsymbol{u}),d\bigr]\,\mathrm{d} \Omega - \int_{\partial\Omega_t } \boldsymbol{t}_{N} \cdot \boldsymbol{u} \,\mathrm{d}A - \int_{\Omega} \boldsymbol{b} \cdot \boldsymbol{u}\,\mathrm{d} \Omega +  \int_{\Omega} G_c \gamma (d, \nabla d) ~\mathrm{d}\Omega,
    \end{aligned}
\end{equation}
where $d:\Omega\rightarrow[0,1]$ represents the phase field, characterizing the material at its pristine state with $d = 0$ and at the fully damaged state with $d = 1$. Also, $\boldsymbol{t}_{N}:\partial\Omega_t\rightarrow\mathbb{R}^n$ is the prescribed traction boundary condition{,} and $ \boldsymbol{b}:\Omega\rightarrow\mathbb{R}^n$ is the body force. The strain energy density takes the following form 
\begin{equation}\label{Eq:strain_energy_density}
    \begin{aligned}
        \varPsi\bigl[\bm{\varepsilon},d\bigr] = g(d)\varPsi^\text{t}(\bm{\varepsilon}^\text{t}) + \varPsi^\text{c}(\bm{\varepsilon}^\text{c}),
    \end{aligned}
\end{equation}
where $g(d)=(1-d)^2$ is a degradation function. 
% and $\varPsi^\text{t}$ and $\varPsi^\text{c}$ are, respectively, the crack-driving and persistent portions of the strain energy density, later we provide more details.
Furthermore, $ G_c > 0 $ is the critical crack energy release rate, and $\gamma(d,\nabla d)$ is the crack surface density per unit volume,
\begin{equation*}
     \gamma(d,\nabla d) = 
     \frac{1}{4c_w}\left( \frac{w(d)}{\ell}+\ell |\nabla d|^2 \right),
\end{equation*}
where $ \ell > 0 $ is the regularization length scale parameter which controls the width of the transition region of the smoothed crack. Crack geometric function $w(d)$ and normalization constant $c_w = \int_0^1 \sqrt{w(d)}\,\mathrm{d}d $ are model dependent. Specifically, for brittle fracture, classical examples are $w(d)=d^2$ and $c_w=1/2$ for the \ATtwo{} model; and $w(d)=d$ and $c_w=2/3$ for the \ATone{} model \cite{Pham2011Gradient}. \newline
% In addition, a notable difference between the AT2 and AT1 models is that the former gives rise to a more diffuse phase field profile while the latter generates a phase field profile with a narrow {support} near the crack.
In the sequel we derive the first and second variations of $\Pi_{\ell}$ as in \eqref{Eq:pi}, which will be needed for the discretized formulation. 
\paragraph{First variation of $\Pi_{\ell}$} Taking the first variation yields:
\begin{equation}\label{Eq:first_variation}
    \begin{aligned}
        \delta\Pi[(\bm{u}, d); (\Bar{\bm{u}}, \Bar{d})] &:= \int_{\Omega} %\frac{\partial\varPsi(\boldsymbol{\varepsilon}(\boldsymbol{u}),d)}{\partial\bm{\varepsilon}(\bm{u})}
        \bm{\sigma}\bigl[\bm{\varepsilon}(\bm{u}), d\bigr]
        \cdot\bm{\varepsilon}(\Bar{\bm{u}})\,\mathrm{d} \Omega 
        - \int_{\partial\Omega_t } \boldsymbol{t}_{N} \cdot \Bar{\boldsymbol{u}} \,\mathrm{d}A 
        - \int_{\Omega} \boldsymbol{b} \cdot \Bar{\boldsymbol{u}}\,\mathrm{d} \Omega \\
        &+ \int_{\Omega} g^{\prime}(d) \varPsi^\text{t}(\boldsymbol{\varepsilon})\Bar{d} ~\mathrm{d}\Omega 
        + \frac{G_c}{4c_w} \int_{\Omega} \Bigl(\frac{w^{\prime}(d)\Bar{d}}{\ell} + 2\ell \nabla d \cdot \nabla \Bar{d} \Bigr) ~\mathrm{d}\Omega,
    \end{aligned}
\end{equation}
where 
\begin{equation}\label{Eq:sigma_degraded}
    \begin{aligned}
        \bm{\sigma} := \frac{\partial\varPsi}{\partial\bm{\varepsilon}} = g(d)\bm{\sigma}^\text{t} + \bm{\sigma}^\text{c}, \quad \bm{\sigma}^\text{t} = \frac{\partial\varPsi^\text{t}}{\partial\bm{\varepsilon}}, \quad \bm{\sigma}^\text{c} = \frac{\partial\varPsi^\text{c}}{\partial\bm{\varepsilon}}.
    \end{aligned}
\end{equation}
\paragraph{Second variation of $\Pi_{\ell}$} We take another variation from \eqref{Eq:pi}:
\begin{equation}\label{Eq:second_variation}
    \begin{aligned}
        \delta^2\Pi[(\bm{u}, d); (\Bar{\bm{u}}, \Bar{d}); (\delta\bm{u}, \delta d)] &:= \int_{\Omega} 
        \bm{\varepsilon}(\delta\bm{u})\cdot\mathbb{C}\bigl[\bm{\varepsilon}(\bm{u}), d \bigr] \cdot \bm{\varepsilon}(\Bar{\bm{u}})\,\mathrm{d} \Omega 
        + \int_{\Omega} \bm{\varepsilon}(\delta\bm{u})\cdot \bm{\sigma}^\text{t}\bigl[\bm{\varepsilon}(\bm{u})\bigr] g^{\prime}(d)\Bar{d}\,\mathrm{d} \Omega \\
        &+ \int_{\Omega} \delta d g^{\prime}(d) \bm{\sigma}^\text{t}\bigl[\bm{\varepsilon}(\bm{u})\bigr]\cdot \bm{\varepsilon}(\Bar{\bm{u}}) \,\mathrm{d} \Omega
        + \int_{\Omega} \delta d g^{\prime\prime}(d)\varPsi^\text{t}(\bm{\varepsilon}) \Bar{d} \,\mathrm{d} \Omega \\
        &+ \frac{g_c}{4c_w} \int_{\Omega} \Biggl(\frac{\delta d w^{\prime\prime}(d) \Bar{d}}{\ell} + 2\ell\nabla(\delta d) \cdot \nabla\Bar{d} \Biggr) \,\mathrm{d} \Omega,
    \end{aligned}
\end{equation}
where 
\begin{equation}\label{Eq:C_degraded}
    \begin{aligned}
        \mathbb{C} := \frac{\partial^2\varPsi}{\partial\bm{\varepsilon}^2} = g(d) \mathbb{C}^\text{t} + \mathbb{C}^\text{c}, \quad \mathbb{C}^\text{t} = \frac{\partial^2\varPsi^\text{t}}{\partial\bm{\varepsilon}^2}, \quad \mathbb{C}^\text{c} = \frac{\partial^2\varPsi^\text{c}}{\partial\bm{\varepsilon}^2}.
    \end{aligned}
\end{equation}
% \paragraph{Residual matrices}
% The residual matrices form of \eqref{Eq:first_variation} are obtained as follows:
% \begin{subequations}\label{Eq:residual_matrices}
%     \begin{align}
%         \bm{R}_A = \int_{\Omega} (\undertilde{\bm{B}_A})^\text{T} \undertilde{\bm{\sigma}}\bigl[\bm{\varepsilon}(u), d\bigr] \,\mathrm{d} \Omega 
%         - \int_{\partial\Omega_t } (\undertilde{\bm{N}_A})^\text{T} \undertilde{\boldsymbol{t}_{N}} \,\mathrm{d}A 
%         - \int_{\Omega} (\undertilde{\bm{N}_A})^\text{T} \undertilde{\boldsymbol{b}} \, \mathrm{d} \Omega, \\
%         \Bar{\bm{R}}_P = \int_{\Omega} g^{\prime}(d)\varPsi^\text{t}(\bm{\varepsilon}) N_P \,\mathrm{d} \Omega 
%         + \frac{g_c}{4c_w} \int_{\Omega} \Biggl(\frac{w^{\prime}(d)N_P}{\ell} + 2 \ell \nabla d \cdot \nabla N_P \Biggr) \,\mathrm{d} \Omega,
%     \end{align}
% \end{subequations}
% where $\bm{R}_A \in \mathbb{R}^n$ and $\Bar{\bm{R}}_P \in \mathbb{R}$ represent the residual entries obtained with displacement test function and phase field test function, respectively.
% Note that $\undertilde{\bm{B}_A}$ is the strain-displacement matrix.
% \paragraph{tangent stiffness matrices}
% The tangent stiffness matrices form of \eqref{Eq:second_variation} are given by
% \begin{subequations}
%     \begin{align}
%         \bm{K}_{AB} &= \int_{\Omega} (\undertilde{\bm{B}_A})^\text{T}\undertilde{\bm{D}}\undertilde{\bm{B}_B} ~\mathrm{d}\Omega, \\
%         \Bar{K}_{PQ} &= \int_{\Omega} g^{\prime\prime}(d) \varPsi^\text{t}(\bm{\varepsilon}) N_P N_Q ~\mathrm{d}\Omega 
%         + \frac{g_c}{4c_w} \int_{\Omega} \Biggl(\frac{w^{\prime\prime}(d)N_P N_Q}{\ell} + 2\ell \nabla N_P \cdot \nabla N_Q \Biggr) \,\mathrm{d} \Omega,    
%     \end{align}
% \end{subequations}
% where $\undertilde{\bm{D}}$ is the matrix form of $\mathbb{C}$ as in \eqref{Eq:C_degraded}.
The components of \eqref{Eq:strain_energy_density}, \eqref{Eq:sigma_degraded}, \eqref{Eq:C_degraded} are particularly obtained in the sequel.
\subsection{Transformation for anisotropic $\mathbb{C}$}\label{Sec:problem-transformation}
% We let the strain decomposition be orthogonal so that $\bm{\varepsilon}^\text{t}\cdot\bm{\varepsilon}^\text{c}=0$. When $\mathbb{C}$ is anisotropic, the orthogonality condition \eqref{Eq:orthogonality} does not hold anymore, i.e., \[\mathbb{C}\bigl(\bm{\varepsilon}^\text{t}\cdot\bm{\varepsilon}^\text{c}\bigr) \neq 0.\] Therefore, 
Let $\mathcal{S}$ and $\mathcal{S}^*$ be the set of all second-order strain and stress tensors, respectively. To enforce the orthogonality condition \eqref{Eq:orthogonality} for an arbitrary anisotropic $\mathbb{C}$, following He and Shao \cite{He-2019}, we define the transformed strain and stress spaces as
%\TNtodo{changed to compliance for stress mapping}
\begin{subequations}\label{Eq:all_transf}
    \begin{align}
        \tilde{\mathcal{S}}=\Big\{\tilde{\bm{\varepsilon}}\Big|\tilde{\bm{\varepsilon}}=\mathbb{C}^{1/2}\bm{\varepsilon},~\bm{\varepsilon}\in\mathcal{S}\Big\}, \label{Eq:eps_transf}\\
        {\tilde{\mathcal{S}}}^*=\Big\{\tilde{\bm{\sigma}}\Big|\tilde{\bm{\sigma}}=\mathbb{S}^{1/2}\bm{\sigma},~\bm{\sigma}\in\mathcal{S}^*\Big\}, \label{Eq:sigma_transf}
    \end{align}
\end{subequations}
so that
\begin{equation}\label{Eq:psi_tilde_decomp}
    \begin{aligned}
        \varPsi(\bm{\varepsilon}) = \frac12 \tilde{\bm{\varepsilon}}\cdot\tilde{\bm{\varepsilon}} = \frac12 \tilde{\bm{\sigma}}\cdot\tilde{\bm{\sigma}}.
    \end{aligned}
\end{equation}
% \TNtodoi{... so that
% \begin{equation}
%     \psi = \frac{1}{2}\tilde{\boldsymbol{\varepsilon}} \dcdot \tilde{\boldsymbol{\varepsilon}} = \frac{1}{2}\tilde{\boldsymbol{\sigma}} \dcdot \tilde{\boldsymbol{\sigma}}
% \end{equation}
% }
{Note that $\mathbb{C}^{1/2}$ in \eqref{Eq:eps_transf} is the square root of $\mathbb{C}$, and $\mathbb{S}^{1/2}$ in \eqref{Eq:sigma_transf} is the square root of the compliance tensor $\mathbb{S}=\mathbb{C}^{-1}$, see Remark \eqref{Re:C_squar} for how to compute $\mathbb{C}^{1/2}$.}
Now let $\tilde{\mathcal{S}}$ and ${\tilde{\mathcal{S}}}^*$ be split into two convex subsets such that
\begin{subequations}\label{Eq:S-st-split}
    \begin{align}
        \tilde{\mathcal{S}}={\tilde{\mathcal{S}}}^{t} \cup {\tilde{\mathcal{S}}}^{c}, \label{Eq:S-st-split-strain} \\
        {\tilde{\mathcal{S}}}^*={\tilde{\mathcal{S}}}^{*t} \cup {\tilde{\mathcal{S}}}^{*c}. \label{Eq:S-st-split-stress}
    \end{align}
\end{subequations}
\eqref{Eq:S-st-split-strain} means that any element $\tilde{\bm{\varepsilon}}\in\tilde{\mathcal{S}}$ is decomposed into a crack-driving portion $\tilde{\bm{\varepsilon}}^{t}$ and a persistent portion $\tilde{\bm{\varepsilon}}^{c}$ such that
\begin{equation}\label{Eq:eps_tild_cond}
    \begin{aligned}
        \tilde{\bm{\varepsilon}} = \tilde{\bm{\varepsilon}}^\text{t} + \tilde{\bm{\varepsilon}}^\text{c}, \quad
        \tilde{\bm{\varepsilon}}^\text{t}\cdot\tilde{\bm{\varepsilon}}^\text{c}=0.
    \end{aligned}
\end{equation}
Similarly for the stress, one writes
\begin{equation*}
    \begin{aligned}
        \tilde{\bm{\sigma}} = \tilde{\bm{\sigma}}^\text{t} + \tilde{\bm{\sigma}}^\text{c}, \quad
        \tilde{\bm{\sigma}}^\text{t}\cdot\tilde{\bm{\sigma}}^\text{c}=0.
    \end{aligned}
\end{equation*}
Thus, with reference to \eqref{Eq:psi_tilde_decomp} the strain energy in the transformed spaces $\tilde{\mathcal{S}}$ or ${\tilde{\mathcal{S}}}^*$ can be decomposed as:
\begin{equation}\label{Eq:psi_tild_split}
    \begin{aligned}
        \varPsi(\tilde{\bm{\varepsilon}}) = \frac12\tilde{\bm{\varepsilon}}^\text{t}\cdot\tilde{\bm{\varepsilon}}^\text{t} + \frac12 \tilde{\bm{\varepsilon}}^\text{c}\cdot\tilde{\bm{\varepsilon}}^\text{c}, \quad
        \varPsi(\tilde{\bm{\sigma}}) = \frac12\tilde{\bm{\sigma}}^\text{t}\cdot\tilde{\bm{\sigma}}^\text{t} + \frac12 \tilde{\bm{\sigma}}^\text{c}\cdot\tilde{\bm{\sigma}}^\text{c}.
    \end{aligned}
\end{equation}
% A similar procedure can be followed to rewrite $\varPsi$ in terms of transformed stress $\tilde{\bm{\sigma}}\in\tilde{\mathcal{K}}_{\sigma}$:
% \begin{equation*}
%     \begin{aligned}
%         \varPsi(\tilde{\bm{\sigma}}) = \frac12\tilde{\bm{\sigma}}^\text{t}\cdot\tilde{\bm{\sigma}}^\text{t} + \frac12 \tilde{\bm{\sigma}}^\text{c}\cdot\tilde{\bm{\sigma}}^\text{c}.
%     \end{aligned}
% \end{equation*}
With $\tilde{\bm{\varepsilon}}^\text{t}$ and $\tilde{\bm{\varepsilon}}^\text{c}$ obtained, one can determine the inverse transformations:
\begin{equation}\label{Eq:tilde_ortho_cond}
    \begin{aligned}
        {\boldsymbol{\varepsilon}}^{t}=\mathbb{C}^{-1/2}\tilde{\boldsymbol{\varepsilon}}^{t}, \quad {\boldsymbol{\varepsilon}}^{c}=\mathbb{C}^{-1/2}\tilde{\boldsymbol{\varepsilon}}^{c}.
    \end{aligned}
\end{equation}
And similarly for the stress:
\begin{equation*}
    \begin{aligned}
        \bm{\sigma}^\text{t} = \mathbb{S}^{-1/2}\tilde{\bm{\sigma}}^\text{t}, \quad \bm{\sigma}^\text{c} = \mathbb{S}^{-1/2}\tilde{\bm{\sigma}}^\text{c}.
    \end{aligned}
\end{equation*}
% With the re-transformation in \eqref{Eq:tilde_ortho_cond}, 
% one can write \[\mathcal{K}=\mathcal{K}^\text{t} + \mathcal{K}^\text{c}, \quad \mathcal{K}=\mathcal{K}^\text{t} + \mathcal{K}^\text{c},\] where the convex subsets of $\mathcal{K}$ read:
% \begin{subequations}
%     \begin{align}
%         \mathcal{K}^{t}=\Big\{\boldsymbol{\varepsilon}^{t}\Big|\boldsymbol{\varepsilon}^{t}=\mathbb{C}^{-1/2}\tilde{\boldsymbol{\varepsilon}}_{\pm},~\tilde{\boldsymbol{\varepsilon}}_{\pm}\in\tilde{\mathcal{K}}_{\pm}\Big\}.
%     \end{align}
% \end{subequations}
% In other words, for any element $\boldsymbol{\varepsilon}\in\mathcal{E}$, there exist $\boldsymbol{\varepsilon}_{\pm}\in\mathcal{K}_{\pm}$ such that \eqref{Eq:orthogonality} holds.
% This way, we satisfy the set of equations in \eqref{Eq:governing}. Then, we can write
% \begin{subequations}\label{Eq:K_decmp}
%     \begin{align}
%         \mathcal{K}_{\varepsilon} = \mathcal{K}_{\varepsilon}^\text{t} + \mathcal{K}_{\varepsilon}^\text{c}, \\
%         \mathcal{K}_{\sigma} = \mathcal{K}_{\sigma}^\text{t} + \mathcal{K}_{\sigma}^\text{c},
%     \end{align}
% \end{subequations}
% where the convex subsets of $\mathcal{K}_{\varepsilon}$ and $\mathcal{K}_{\sigma}$ are obtained by:
One can observe that orthogonality also holds for the quantities transformed back to the physical stress and strain spaces.
Henceforth, the convex subsets are summarized as follows:
\begin{subequations}\label{Eq:S-tc-remap}
    \begin{align}
        \mathcal{S}^\text{t}=\Big\{\bm{\varepsilon}^\text{t}\Big|\bm{\varepsilon}^\text{t}=\mathbb{C}^{-1/2}\tilde{\bm{\varepsilon}}^\text{t},~\tilde{\bm{\varepsilon}}^\text{t}\in{\tilde{\mathcal{S}}}^{t}\Big\}, \quad \mathcal{S}^\text{c}=\Big\{\bm{\varepsilon}^\text{c}\Big|\bm{\varepsilon}^\text{c}=\mathbb{C}^{-1/2}\tilde{\bm{\varepsilon}}^\text{c},~\tilde{\bm{\varepsilon}}^\text{c}\in{\tilde{\mathcal{S}}}^{c}\Big\}, \label{Eq:S-tc-remap-strain} \\
        \mathcal{S}^{*t}=\Big\{\bm{\sigma}^\text{t}\Big|\bm{\sigma}^\text{t}=\mathbb{S}^{-1/2}\tilde{\bm{\sigma}}^\text{t},~\tilde{\bm{\sigma}}^\text{t}\in{\tilde{\mathcal{S}}}^{*t}\Big\}, \quad
        \mathcal{S}^{*c}=\Big\{\bm{\sigma}^\text{c}\Big|\bm{\sigma}^\text{c}=\mathbb{S}^{-1/2}\tilde{\bm{\sigma}}^\text{c},~\tilde{\bm{\sigma}}^\text{c}\in{\tilde{\mathcal{S}}}^{*c}\Big\}. \label{Eq:S-tc-remap-stress}
    \end{align}
\end{subequations}
\begin{remark}\label{Re:C_squar}
We derive the square root of $\mathbb{C}$ as follows. As $\mathbb{C}$ has major symmetry and is positive-definitive, one can write its spectral decomposition as below:
\begin{equation*}
    \begin{aligned}
        \mathbb{C}=\underset{i}{\sum}\Lambda_i~\textbf{\textomega}_i\otimes\textbf{\textomega}_i,
    \end{aligned}
\end{equation*}
where $\Lambda_i>0$ are the eigenvalues of $\mathbb{C}$ and \textbf{\textomega}$_i$ are the second-order orthonormal eigentensors associated to $\Lambda_i$, such that $\textbf{\textomega}_i\cdot\textbf{\textomega}_j=\delta_{ij}$.
Then, we can compute the square root of $\mathbb{C}$ by:
\begin{equation}\label{Eq:C_spectral_decomp}
    \begin{aligned}
        \mathbb{C}^{1/2}=\underset{i}{\sum}\Lambda_i^{1/2}\textbf{\textomega}_i\otimes\textbf{\textomega}_i.
    \end{aligned}
\end{equation}
% It is worth noting that $\mathbb{C}^{1/2}$ and $\mathbb{C}^{-1/2}$ have to be evaluated only once during the simulation.
The same procedure can be followed for the compliance tensor $\mathbb{S}$.
\end{remark}
\paragraph*{Summary of \ref{Sec:problem-transformation}} {We aimed at satisfying the orthogonality condition \eqref{Eq:orthogonality} for anisotropic $\mathbb{C}$. We illustrated that for any $\bm{\varepsilon}\in\mathcal{S}$, there exist $\bm{\varepsilon}^\text{t}\in\mathcal{S}^{t}$ and $\bm{\varepsilon}^\text{c}\in\mathcal{S}^{c}$ such that the orthogonality condition holds. This was achieved through an energy preserving transformation ($\varPsi(\bm{\varepsilon}) = \varPsi(\tilde{\bm{\varepsilon}})$) to a new space $\tilde{\bm{\varepsilon}}\in\tilde{\mathcal{S}}$ where $\varPsi(\tilde{\bm{\varepsilon}}) = \varPsi(\tilde{\bm{\varepsilon}}^\text{t}) + \varPsi(\tilde{\bm{\varepsilon}}^\text{c})$. The remaining step is to make a choice for $\tilde{\mathcal{S}}^\text{t}$ and $\tilde{\mathcal{S}}^\text{c}$ and derive the decomposition of the constitutive model, that is, $\varPsi(\bm{\varepsilon}) = \varPsi(\bm{\varepsilon}^\text{t}) + \varPsi(\bm{\varepsilon}^\text{c})$.}
\subsection{Choice of tension-compression asymmetry}\label{Sec:problem-unilateral}
% The choice of the convex subsets ${\tilde{\mathcal{S}}}^\text{t}$ and ${\tilde{\mathcal{S}}}^\text{c}$ as in \eqref{Eq:S-st-split-strain} is not unique and has to be made according to what we mean by `crack-driving' and `persistent' in a three-dimensional setting. Note that the requirement that ${\tilde{\mathcal{S}}}^\text{t}$ and ${\tilde{\mathcal{S}}}^\text{c}$ be convex ensures the uniqueness of the projection of any given transformed strain tensor $\tilde{\boldsymbol{\varepsilon}}\in\tilde{\mathcal{S}}$ on ${\tilde{\mathcal{S}}}^\text{t}$ and ${\tilde{\mathcal{S}}}^\text{c}$. Once ${\tilde{\mathcal{S}}}^\text{t}$ and ${\tilde{\mathcal{S}}}^\text{c}$ are decided, we can derive ${\mathcal{S}}^\text{t}$ and ${\mathcal{S}}^\text{c}$ according to \eqref{Eq:S-tc-remap-strain}.
% \KYtodoi{Mention though the spectral decomposition is one of the most popular split, we cannot use it here because it does not meet the orthogonality. VZ: Done in the abstract}
Several existing models for tension-compression asymmetry can be derived in accordance with the variational principle in \eqref{Eq:variational_principle}. Here, we list a few choices:
\begin{itemize}
    \item The original model proposed by Bourdin et al. \cite{Bourdin2000} adopts a symmetric response of the cracked solid, i.e., it assumes that both tension and compression loads contribute equally to cracking. If $\tilde{\mathcal{S}}^\text{t}$ is taken as the set of all symmetric second-order tensors, this model is retrieved.
    \item The volumetric-deviatoric by Amor et al. \cite{Amor2009} assumes that both volumetric expansion and deviatoric deformation contribute to crack propagation but not volumetric compression. $\tilde{\mathcal{S}}^\text{t}$ represents all symmetric second-order tensors with a non-negative trace ($\tr{\tilde{\bm{\varepsilon}}}\geq 0$), i.e. volumetric expansion.
    \item The no-tension by Freddi and Royer-Carfagni \cite{Freddi2010} is a model for masonry-like materials that accounts for the Poisson effect. This model is retrieved when $\tilde{\mathcal{S}}^\text{t}$ is chosen to be the set of all positive semi-definite symmetric tensors. The stress attained at a fully damaged material point is negative semi-definite, which corresponds to the fact that the material does not support tension.
\end{itemize}
    \begin{remark}\label{Re:Intro_Miehe}
        % The positive part of the strain minimizes the negative part of the elastic energy that resists to damage. 
        % \deleted[id=VZR]{However, it is well known that in certain tests, unphysical predictions are resulted, e.g. bending test with the VD split and through-crack shear test with the spectral decomposition.}
        % The masonry-like model \cite{Freddi2010} corresponds in fact to the materials that do not support tension.
        % Recently, more sophisticated models based on the local crack orientation were proposed. For example, in the two models by Strobl and Seelig \cite{Strobl2015}, the crack orientation is assumed to coincide with the local gradient direction of the phase field. Both models are variationally inconsistent though. Liu et al. \cite{LIU2021} proposeed a \dots \newline
        Not all existing approaches that account for the tension-compression asymmetry satisfy the variational principle. For instance, the well known spectral-decomposition model by Miehe et al. \cite{Miehe2010} adopts the elastic energy density split as below, but does not fit into the variational formalism:
        \begin{equation*}
            \begin{aligned}
                \varPsi(\bm{\varepsilon}) &= \varPsi^\text{t}(\bm{\varepsilon}) + \varPsi^\text{c}(\bm{\varepsilon}), \\
                \varPsi^{t}(\bm{\varepsilon}) &= \frac12 \lambda \langle \tr{\bm{\varepsilon}} \rangle_{+} + \mu \bm{\varepsilon}^{t} \cdot \bm{\varepsilon}^{t}, \quad
                \varPsi^{c}(\bm{\varepsilon}) = \frac12 \lambda \langle \tr{\bm{\varepsilon}} \rangle_{-} + \mu \bm{\varepsilon}^{c} \cdot \bm{\varepsilon}^{c},
                % \varPsi^{t|c}(\bm{\varepsilon}) = \frac12 \lambda \langle \tr{\bm{\varepsilon}} \rangle_{\pm} + \mu \bm{\varepsilon}^{t|c} \cdot \bm{\varepsilon}^{t|c}, \\
                % \bm{\sigma}(\bm{\varepsilon}) = \bm{\sigma}^\text{t}(\bm{\varepsilon}) + \bm{\sigma}^\text{c}(\bm{\varepsilon}), \quad \bm{\sigma}^{t|c}(\bm{\varepsilon}) = \lambda \langle \tr{\bm{\varepsilon}}\rangle_{\pm} \bm{1} + 2\mu \bm{\varepsilon}^{t|c},
            \end{aligned}
        \end{equation*}
        where the Macaulay bracket is defined as $\langle\cdot\rangle_{\pm} := (\cdot\pm \lvert\cdot\rvert)/2$, and $\bm{\varepsilon}^{t}$, $\bm{\varepsilon}^{c}$ are obtained by projecting $\bm{\varepsilon}$ onto the space of all symmetric positive/negative semi-definite tensors with respect to the Frobenius norm. Here, contrary to our recent assumption, the constitutive relations cannot be partitioned based on merely $\bm{\varepsilon}^\text{t}$ or $\bm{\varepsilon}^\text{c}$. 
        % Despite its variational inconsistency, the stress for a totally damaged element is also negative semi-definite as for {no-tension}. {However, Li et al. \cite{Marigo2016} reported some different behavior under compression for spectral-decomposition and {no-tension}.} 
        Consequently, one can not adopt the spectral-decomposition model in the variational formalism. \newline
        % while Miehe et al. \cite{Freddi2010} based their model on the spectral decomposition of the strain tensor.
    \end{remark}
In the following, we provide implementation details of our model based on two choices: (a) {volumetric-deviatoric} and (b) {no-tension}. This means $\tilde{\mathcal{S}}$ can be split into two portions accordingly.
\subsubsection{Volumetric-deviatoric}
%  model by Amor et al. \cite{Amor2009}
We split the transformed strain into volumetric and deviatoric parts,
%{This split suggests to decompose the strain tensor into a volumetric and a deviatoric part as follows:}{This split is based on the assumption that the strain energy resulting in the decrease of the local volume will not be degraded.}
\begin{subequations}\label{Eq:Amor_split}
    \begin{align}
        {\tilde{\mathcal{S}}}^\text{t}=\Big\{\tilde{\bm{\varepsilon}}\in\tilde{\mathcal{S}}\Big|\tr({\tilde{\bm{\varepsilon}}})\geq 0\Big\}, \\
        {\tilde{\mathcal{S}}}^\text{c}=\Big\{\tilde{\bm{\varepsilon}}\in\tilde{\mathcal{S}}\Big|\tilde{\bm{\varepsilon}}=a\mathbf{1},~a \leq 0\Big\},
    \end{align}
\end{subequations}
where $\mathbf{1}$ is the second-order identity tensor. 
Thus, the strain in the transformed space is decomposed as follows:
\begin{subequations}\label{Eq:Amor_decomp}
    \begin{align}
        \tilde{\boldsymbol{\varepsilon}}^{t} = \frac13\langle\tr{\tilde{\boldsymbol{\varepsilon}}}\rangle_{+}\mathbf{1} 
        + \dev\tilde{\boldsymbol{\varepsilon}},\\
        \tilde{\boldsymbol{\varepsilon}}^{c} = \frac13\langle\tr{\tilde{\boldsymbol{\varepsilon}}}\rangle_{-}\mathbf{1},
    \end{align}
\end{subequations}
where $\dev\tilde{\boldsymbol{\varepsilon}} = \tilde{\boldsymbol{\varepsilon}} - \frac13 (\tr{\tilde{\boldsymbol{\varepsilon}}})\textbf{1}.$
% Using Kelvin notation\TNtodo{likewise: $[\sigma_{ij}]$, etc.}\dcdot
Note that this partitioning satisfies \eqref{Eq:eps_tild_cond}.
\subsubsection*{Decomposition of constitutive model}
The derivatives of $\tilde{\boldsymbol{\varepsilon}}^{t}$ and $\tilde{\boldsymbol{\varepsilon}}^{c}$ with respect to 
% the transformed strain tensor 
$\tilde{\boldsymbol{\varepsilon}}$ define two projection tensors as:
\begin{subequations}\label{Eq:D_tensors}
    \begin{align}
        \mathbb{D}^\text{t} := \frac{\partial\tilde{\bm{\varepsilon}}^\text{t}}{\partial\tilde{\bm{\varepsilon}}} = \frac13 H\bigl[\tr{(\mathbb{C}^{1/2}\boldsymbol{\varepsilon})}\bigr]\mathbf{1}\otimes\mathbf{1}
        + \Bigl(\mathds{1}-\frac13\mathbf{1}\otimes\mathbf{1}\Bigr),\\
        \mathbb{D}^\text{c} := \frac{\partial\tilde{\bm{\varepsilon}}^\text{c}}{\partial\tilde{\bm{\varepsilon}}} = \frac13 H\bigl[-\tr{(\mathbb{C}^{1/2}\boldsymbol{\varepsilon})}\bigr]\mathbf{1}\otimes\mathbf{1},
    \end{align}
\end{subequations}
where $\mathds{1}$ is the fourth-order identity tensor, and $H$ is the Heaviside function such that $H(a) = 1$ if $a\geq 0$, and $H(a)=0$ otherwise.
% \deleted[]{, also $H(a)=1/2$ if $a=0$ for sake of symmetry}. \KYtodo{Really? VZ: I planned to, but haven't implemented it though.)} \newline
Then, by applying the chain rule, we obtain:
\begin{equation*}
    \begin{aligned}
        % \frac{\partial\bm{\varepsilon}^\text{t}}{\partial\bm{\varepsilon}}=\mathbb{C}^{-1/2}\Bigl(\frac{\partial\tilde{\bm{\varepsilon}}^{t}}{\partial\tilde{\bm{\varepsilon}}}\Bigr)\mathbb{C}^{1/2},
        \frac{\partial\bm{\varepsilon}^\text{t}}{\partial\bm{\varepsilon}}=\mathbb{C}^{-1/2}\mathbb{D}^\text{t}\mathbb{C}^{1/2},
        % \quad \frac{\partial\bm{\varepsilon}^\text{c}}{\partial\bm{\varepsilon}}=\mathbb{C}^{-1/2}\Bigl(\frac{\partial\tilde{\bm{\varepsilon}}^{c}}{\partial\tilde{\bm{\varepsilon}}}\Bigr)\mathbb{C}^{1/2}.
        \quad \frac{\partial\bm{\varepsilon}^\text{c}}{\partial\bm{\varepsilon}}=\mathbb{C}^{-1/2}\mathbb{D}^\text{c}\mathbb{C}^{1/2}.
    \end{aligned}
\end{equation*}
Therefore, the decomposition of ${\boldsymbol{\varepsilon}}$ into ${\boldsymbol{\varepsilon}}^{t}~\text{and}~{\boldsymbol{\varepsilon}}^{c}$ reads:
\begin{subequations}\label{Eq:strain_decomp_voldev}
    \begin{align}
        % \boldsymbol{\varepsilon}^{t} &= \Bigl(\mathbb{C}^{-1/2}\dcdot\Big\{\frac13 H(\tr{\tilde{\boldsymbol{\varepsilon}}})\mathbf{1}\otimes\mathbf{1} +\bigl(\mathds{1}-\frac13\mathbf{1}\otimes\mathbf{1}\bigr)\Big\}\dcdot\mathbb{C}^{1/2}\Bigr)\dcdot\boldsymbol{\varepsilon},\\
        \boldsymbol{\varepsilon}^{t} &= \Bigl(\mathbb{C}^{-1/2}\mathbb{D}^\text{t}\mathbb{C}^{1/2}\Bigr)\boldsymbol{\varepsilon},\\
        % \boldsymbol{\varepsilon}^{c} &= \Bigl(\mathbb{C}^{-1/2}\dcdot\Big\{\frac13 H(-\tr{\tilde{\boldsymbol{\varepsilon}}})\mathbf{1}\otimes\mathbf{1}\Big\}\dcdot\mathbb{C}^{1/2}\Bigr)\dcdot\boldsymbol{\varepsilon}.
        \boldsymbol{\varepsilon}^{c} &= \Bigl(\mathbb{C}^{-1/2}\mathbb{D}^\text{c}\mathbb{C}^{1/2}\Bigr)\boldsymbol{\varepsilon}.
    \end{align}
\end{subequations}
Moreover, we derive the stress decomposition as:
\begin{equation}\label{Eq:sigma}
    \begin{aligned}
        \bm{\sigma}^\text{t} := \frac{\partial\varPsi^\text{t}}{\partial\bm{\varepsilon}} = \mathbb{C}\bm{\varepsilon}^\text{t}
        % \deleted[id=VZR]{\frac{\partial\bm{\varepsilon}^\text{t}}{\partial\bm{\varepsilon}}} 
        = \mathbb{C}^\text{t}\bm{\varepsilon}, \quad \bm{\sigma}^\text{c} := \frac{\partial\varPsi^\text{c}}{\partial\bm{\varepsilon}} = \mathbb{C}\bm{\varepsilon}^\text{c}
        % \deleted[id=VZR]{\frac{\partial\bm{\varepsilon}^\text{c}}{\partial\bm{\varepsilon}}} 
        = \mathbb{C}^\text{c}\bm{\varepsilon}.
    \end{aligned}
\end{equation}
On this basis, we can also split $\mathbb{C}=\frac{\partial^2\varPsi}{\partial\bm{\varepsilon}^2}$ into two portions \[\mathbb{C} = \mathbb{C}^\text{t} + \mathbb{C}^\text{c},\]
where $\mathbb{C}^{t}$ and $\mathbb{C}^\text{c}$ are respectively,
%\TNtodo{"as $\partial^2 \varPsi_\pm / \partial\boldsymbol\varepsilon^2$"?}\VZRtodo{yes. i will rewrite this part, and perhaps add more intermediate steps as well.}:
\begin{subequations}\label{Eq:C_decomp}
    \begin{align}
        \mathbb{C}^{t} := \frac{\partial^2 \varPsi^\text{t}}{\partial\bm{\varepsilon}^2} = \bigl(\frac{\partial\bm{\varepsilon}^\text{t}}{\partial{\boldsymbol{\varepsilon}}}\bigr)^\text{T}\mathbb{C}\frac{\partial\bm{\varepsilon}^\text{t}}{\partial{\boldsymbol{\varepsilon}}},\\
        % \mathbb{C}^{t} = \frac{\partial^2 \varPsi^\text{t}}{\partial\bm{\varepsilon}^2} = (\mathbb{C}^{1/2})^\text{T}\mathbb{D}^\text{t}\mathbb{C}^{1/2},\\
        \mathbb{C}^{c} := \frac{\partial^2 \varPsi^\text{c}}{\partial\bm{\varepsilon}^2} = \bigl(\frac{\partial\bm{\varepsilon}^\text{c}}{\partial{\boldsymbol{\varepsilon}}}\bigr)^\text{T}\mathbb{C}\frac{\partial\bm{\varepsilon}^\text{c}}{\partial{\boldsymbol{\varepsilon}}}.
        % \mathbb{C}^{c} = \frac{\partial^2 \varPsi^\text{c}}{\partial\bm{\varepsilon}^2} = (\mathbb{C}^{1/2})^\text{T}\mathbb{D}^\text{c}\mathbb{C}^{1/2}.
    \end{align}
\end{subequations}
\subsubsection{No-tension}
%  model by Freddi and Royer-Carfagni \cite{Freddi2010}
% such that $\bm{\varepsilon}^\text{t}$ is a positive definite tensor and is coaxial with $\bm{\varepsilon}$ \dots \newline
Taking into account that $\tilde{\bm{\varepsilon}}^\text{t}\cdot\tilde{\bm{\varepsilon}}^\text{c} = 0$, we obtain the following relation for stress-strain in their transformed spaces:
\begin{equation}\label{Eq:mas-isotropy}
    \begin{aligned}
        \tilde{\bm{\sigma}} &:= \frac{\partial\varPsi(\tilde{\bm{\varepsilon}})}{\partial\tilde{\bm{\varepsilon}}} = \frac{\partial}{\partial\tilde{\bm{\varepsilon}}}\Bigl(\frac12\tilde{\bm{\varepsilon}}^\text{t}\cdot\tilde{\bm{\varepsilon}}^\text{t} + \frac12\tilde{\bm{\varepsilon}}^\text{c}\cdot\tilde{\bm{\varepsilon}}^\text{c}\Bigr) = \mathds{1}\tilde{\bm{\varepsilon}}.
    \end{aligned}
\end{equation}
Thus, the stiffness tensor in the transformed spaces is the fourth-order identity tensor, that is, $\tilde{\mathbb{C}}=\frac{\partial\tilde{\bm{\sigma}}}{\partial\tilde{\bm{\varepsilon}}}=\mathds{1}$. On this basis, we can simplify and follow {no-tension} as for the isotropic materials \cite{Freddi2010}. Henceforth, let $(\tilde{\varepsilon}_1, \tilde{\varepsilon}_2, \tilde{\varepsilon}_3)$ be a spectral decomposition of $\tilde{\bm{\varepsilon}}$ such that $\tilde{\varepsilon}_1\geq\tilde{\varepsilon}_2\geq\tilde{\varepsilon}_3$,
\begin{equation}\label{Eq:mas-eps}
    \begin{aligned}
        \tilde{\bm{\varepsilon}} = \overset{3}{\underset{i=1}{\sum}}\tilde{\varepsilon}_i \bm{n}_{(i)} \otimes \bm{n}_{(i)} := \tilde{\varepsilon}_i \bm{M}_i,
    \end{aligned}
\end{equation}
{where $\bm{n}_{(i)}$ represents an eigenvector and parentheses around an index indicate that the usual summation convention is suspended.} 
The strain is decomposed so that $\tilde{\bm{\varepsilon}}^\text{t}$ is a positive definite tensor and is coaxial with $\tilde{\bm{\varepsilon}}$,
\begin{equation}\label{Eq:mas-epspn}
    \begin{aligned}
        \tilde{\bm{\varepsilon}}^{t} = \overset{3}{\underset{i=1}{\sum}} a_i \bm{n}_{(i)} \otimes \bm{n}_{(i)} := a_i \bm{M}_i, \quad \tilde{\bm{\varepsilon}}^{c} = \overset{3}{\underset{i=1}{\sum}} b_i \bm{n}_{(i)} \otimes \bm{n}_{(i)} := b_i \bm{M}_i,
    \end{aligned}
\end{equation}
where $a_i = \langle\tilde{\varepsilon}_i\rangle_{+}$, and $b_i = \tilde{\varepsilon}_i - a_i$. 
% Then, the spectral decomposition of $\tilde{\bm{\varepsilon}}^{t}$ reads:
% \begin{equation}\label{Eq:mas-ai}
%   (a_1, a_2, a_3) =
%     \begin{cases}
%       (\tilde{\varepsilon}_1, \tilde{\varepsilon}_2, \tilde{\varepsilon}_3), & \text{if}~\varepsilon_3 \geq 0 \\
%       (\tilde{\varepsilon}_1, \tilde{\varepsilon}_2, 0), & \text{else if}~ \varepsilon_2 \geq 0 \\
%       (\tilde{\varepsilon}_1, 0, 0), & \text{else if}~ \varepsilon_1\geq 0 \\
%       (0, 0, 0). & \text{otherwise}
%     \end{cases}
% \end{equation}
% Also,
% \begin{equation}\label{Eq:mas-bi}
%     \begin{aligned}
%         (b_1, b_2, b_3) =
%         \begin{cases}
%             (0, 0, 0), & \text{if}~\varepsilon_3 \geq 0 \\
%             (0, 0, \tilde{\varepsilon_3}), & \text{else if}~ \varepsilon_2 \geq 0 \\
%             (0, \tilde{\varepsilon}_2, \tilde{\varepsilon}_3), & \text{else if}~ \varepsilon_1\geq 0 \\
%             (\tilde{\varepsilon}_1, \tilde{\varepsilon}_2, \tilde{\varepsilon}_3). & \text{otherwise}
%         \end{cases}
%     \end{aligned}
% \end{equation}
% \paragraph*{Two-dimensional case} In two-dimensions, \eqref{Eq:mas-eps}, \eqref{Eq:mas-epspn} are modified so that $i$ varies from 1 to 2 and the spectral decomposition of $\tilde{\bm{\varepsilon}}$ reads as ($\tilde{\varepsilon}_1, \tilde{\varepsilon}_2$) such that $\tilde{\varepsilon}_1\geq\tilde{\varepsilon}_2$. Therefore, the spectral decomposition of $\tilde{\bm{\varepsilon}}^\text{t}$ is given by:
% \begin{equation}\label{Eq:mas-ai-2d}
%   (a_1, a_2) =
%     \begin{cases}
%       (\tilde{\varepsilon}_1, \tilde{\varepsilon}_2), & \text{if}~\varepsilon_2 \geq 0 \\
%       (\tilde{\varepsilon}_1, 0), & \text{else if}~ \varepsilon_1 \geq 0 \\
%       (0, 0). & \text{otherwise}
%     \end{cases}
% \end{equation}
% Also,
% \begin{equation}\label{Eq:mas-bi-2d}
%     \begin{aligned}
%         (b_1, b_2) =
%         \begin{cases}
%             (0, 0), & \text{if}~\varepsilon_2 \geq 0 \\
%             (0, \tilde{\varepsilon}_2), & \text{else if}~ \varepsilon_1 \geq 0 \\
%             (\tilde{\varepsilon}_1, \tilde{\varepsilon}_2). & \text{otherwise}
%         \end{cases}
%     \end{aligned}
% \end{equation}
\subsubsection*{Decomposition of constitutive model}
A necessary part is to obtain the derivatives of $\tilde{\bm{\varepsilon}}^\text{t}$ and $\tilde{\bm{\varepsilon}}^\text{c}$ with respect to
% the transformed strain tensor 
$\tilde{\bm{\varepsilon}}$.
\begin{equation}\label{Eq:proj-dir-dev}
    \begin{aligned}
        \mathbb{D}^{t} := \frac{\partial\tilde{\bm{\varepsilon}}^t}{\partial{\tilde{\bm{\varepsilon}}}} &= \overset{3}{\underset{i=1}{\sum}} \frac{\partial a_i}{\partial\tilde{\varepsilon}_i} \bm{n}_{(i)} \otimes \bm{n}_{(i)} \otimes\bm{n}_{(i)} \otimes \bm{n}_{(i)} \\
        &+ \frac12\underset{i\neq j}{\sum} \frac{a_j -a_i}{\tilde{\varepsilon}_j - \tilde{\varepsilon}_i} \Biggl(\bm{n}_{(i)} \otimes \bm{n}_{(j)} \otimes \bm{n}_{(i)} \otimes \bm{n}_{(j)} + \bm{n}_{(i)} \otimes \bm{n}_{(j)} \otimes \bm{n}_{(j)} \otimes \bm{n}_{(i)} \Biggr), \\
        \mathbb{D}^{c} := \frac{\partial\tilde{\bm{\varepsilon}}^c}{\partial{\tilde{\bm{\varepsilon}}}} &= \overset{3}{\underset{i=1}{\sum}} \frac{\partial b_i}{\partial\tilde{\varepsilon}_i} \bm{n}_{(i)} \otimes \bm{n}_{(i)} \otimes\bm{n}_{(i)} \otimes \bm{n}_{(i)} \\
        &+ \frac12 \underset{i\neq j}{\sum} \frac{b_j - b_i}{\tilde{\varepsilon}_j - \tilde{\varepsilon}_i} \Biggl(\bm{n}_{(i)} \otimes \bm{n}_{(j)} \otimes \bm{n}_{(i)} \otimes \bm{n}_{(j)} + \bm{n}_{(i)} \otimes \bm{n}_{(j)} \otimes \bm{n}_{(j)} \otimes \bm{n}_{(i)} \Biggr).
    \end{aligned}
\end{equation}
{For sake of brevity, readers are referred to \ref{App} for a closed-form expression of projection tensors in two-dimensional and three-dimensional settings.} \newline
Similar to {volumetric-deviatoric}, the decomposition of $\bm{\varepsilon}$ can be realized as 
\begin{equation}\label{Eq:strain_decomp_masonry}
    \begin{aligned}
        \boldsymbol{\varepsilon}^{t} = \Bigl(\mathbb{C}^{-1/2}\mathbb{D}^\text{t}\mathbb{C}^{1/2}\Bigr)\boldsymbol{\varepsilon}, \quad
        \boldsymbol{\varepsilon}^{c} = \Bigl(\mathbb{C}^{-1/2}\mathbb{D}^\text{c}\mathbb{C}^{1/2}\Bigr)\boldsymbol{\varepsilon},
    \end{aligned}
\end{equation}
with $\mathbb{D}^\text{t}, \mathbb{D}^\text{c}$ as in \eqref{Eq:proj-dir-dev}. \newline
In addition, we write the stress decomposition as
% \KYtodoi{It would be nice if we explain why we choose this form of the derivatives so that $\mathbb{C}$ expression will not involve higher order tensor derivatives.}
\begin{equation}\label{Eq:sigma_masonry}
    \begin{aligned}
        \sigma^\text{t}_{mn} := \frac{\partial\varPsi^\text{t}}{\partial\varepsilon_{mn}} = \frac{\partial\varPsi^\text{t}}{\partial\tilde{\varepsilon}_{ij}^\text{t}}\frac{\partial\tilde{\varepsilon}_{ij}^\text{t}}{\partial\tilde{\varepsilon}_{kl}}\frac{\partial\tilde{\varepsilon}_{kl}}{\partial\varepsilon_{mn}}=\tilde{\varepsilon}_{ij}^\text{t} D^\text{t}_{ijkl}\mathbb{C}^{1/2}_{klmn} = \tilde{\varepsilon}^\text{t}_{kl} C^{1/2}_{klmn} = C^{1/2}_{mnkl}C^{1/2}_{klpq}{\varepsilon}^\text{t}_{pq}, \\
        \sigma^\text{c}_{mn} := \frac{\partial\varPsi^\text{c}}{\partial\varepsilon_{mn}} = \frac{\partial\varPsi^\text{c}}{\partial\tilde{\varepsilon}_{ij}^\text{c}}\frac{\partial\tilde{\varepsilon}_{ij}^\text{c}}{\partial\tilde{\varepsilon}_{kl}}\frac{\partial\tilde{\varepsilon}_{kl}}{\partial\varepsilon_{mn}}=\tilde{\varepsilon}_{ij}^\text{c} D^\text{c}_{ijkl}\mathbb{C}^{1/2}_{klmn} = \tilde{\varepsilon}^\text{c}_{kl} C^{1/2}_{klmn} = C^{1/2}_{mnkl}C^{1/2}_{klpq}{\varepsilon}^\text{c}_{pq},
    \end{aligned}
\end{equation}
%\KYtodoi{Remark}
or in tensorial form:
\begin{equation}\label{Eq:sigma_masonry_tensor}
    \begin{aligned}
        \bm{\sigma}^\text{t} := \frac{\partial\varPsi^\text{t}}{\partial\bm{\varepsilon}} = \mathbb{C} \bm{\varepsilon}^\text{t}, \quad \bm{\sigma}^\text{c} := \frac{\partial\varPsi^\text{c}}{\partial\bm{\varepsilon}} = \mathbb{C}\bm{\varepsilon}^\text{c}.
    \end{aligned}
\end{equation}
To split $\mathbb{C}=\frac{\partial^2\varPsi}{\partial\bm{\varepsilon}^2}$ into two portions, we take the derivatives of \eqref{Eq:sigma_masonry} as:
\begin{equation}\label{Eq:C_masonry}
    \begin{aligned}
        \frac{\partial^2\varPsi^\text{t}}{\partial\varepsilon_{pq}\partial\varepsilon_{mn}} = \frac{\partial}{\partial\varepsilon_{pq}}\bigl(\tilde{\varepsilon}^\text{t}_{ij}D^\text{t}_{ijkl}\bigr)C^{1/2}_{klmn} = C^{1/2}_{mnkl}\frac{\partial}{\partial\tilde{\varepsilon}_{rs}}\bigl(\tilde{\varepsilon}^\text{t}_{ij}D^\text{t}_{ijkl}\bigr)\frac{\partial\tilde{\varepsilon}_{rs}}{\partial\varepsilon_{pq}} 
        = C^{1/2}_{mnkl}\frac{\partial\tilde{\varepsilon}^\text{t}_{kl}}{\partial\tilde{\varepsilon}_{rs}}\frac{\partial\tilde{\varepsilon}_{rs}}{\partial\varepsilon_{pq}} = C^{1/2}_{mnkl} D^\text{t}_{klrs}C^{1/2}_{rspq}, \\
        \frac{\partial^2\varPsi^\text{c}}{\partial\varepsilon_{pq}\partial\varepsilon_{mn}} = \frac{\partial}{\partial\varepsilon_{pq}}\bigl(\tilde{\varepsilon}^\text{c}_{ij}D^\text{c}_{ijkl}\bigr)C^{1/2}_{klmn} = C^{1/2}_{mnkl}\frac{\partial}{\partial\tilde{\varepsilon}_{rs}}\bigl(\tilde{\varepsilon}^\text{c}_{ij}D^\text{c}_{ijkl}\bigr)\frac{\partial\tilde{\varepsilon}_{rs}}{\partial\varepsilon_{pq}} 
        = C^{1/2}_{mnkl}\frac{\partial\tilde{\varepsilon}^\text{c}_{kl}}{\partial\tilde{\varepsilon}_{rs}}\frac{\partial\tilde{\varepsilon}_{rs}}{\partial\varepsilon_{pq}} = C^{1/2}_{mnkl} D^\text{c}_{klrs}C^{1/2}_{rspq},
    \end{aligned}
\end{equation}
or in tensorial form:
\begin{equation}\label{Eq:C_masonry_tensor}
    \begin{aligned}
        % \mathbb{C}^\text{t} = (\mathbb{C}^{1/2})^\text{T} \mathbb{D}^\text{t} \mathbb{C}^{1/2}, \quad \mathbb{C}^\text{c} = (\mathbb{C}^{1/2})^\text{T} \mathbb{D}^\text{c} \mathbb{C}^{1/2},
        \mathbb{C}^\text{t} = \mathbb{C}^{1/2} \mathbb{D}^\text{t} \mathbb{C}^{1/2}, \quad \mathbb{C}^\text{c} = \mathbb{C}^{1/2} \mathbb{D}^\text{c} \mathbb{C}^{1/2}.
    \end{aligned}
\end{equation}
\begin{remark}\label{Re:tensor_operation}
Note that in \eqref{Eq:sigma_masonry}, $\tilde{\varepsilon}^\text{t}_{ij}D^\text{t}_{ijkl} = \tilde{\varepsilon}^\text{t}_{kl}$ and $\tilde{\varepsilon}^\text{c}_{ij}D^\text{c}_{ijkl} = \tilde{\varepsilon}^\text{c}_{kl}$. This is achieved because of $\frac{\partial a_i}{\partial\tilde{\varepsilon}_i} = H(\tilde{\varepsilon_i})$ and $\frac{\partial b_i}{\partial\tilde{\varepsilon}_i} = H(-\tilde{\varepsilon_i})$ in simplifying \eqref{Eq:proj-dir-dev}. 
Also note in \eqref{Eq:C_masonry} to avoid running into some higher-order tensors, 
rather than employing the product rule, we first compute the aforementioned contractions
% Thus, we first derive the product object, that is, \[\tilde{\varepsilon}_{ij}{D}^\text{t}_{ijkl} = \tilde{\varepsilon}^\text{t}_{kl}, \quad \tilde{\varepsilon}_{ij}{D}^\text{c}_{ijkl} = \tilde{\varepsilon}^\text{c}_{kl},\] 
and thereafter we proceed with taking their derivatives, that is,
\begin{equation*}
    \begin{aligned}
        \frac{\partial}{\partial\tilde{\varepsilon}_{rs}}\bigl(\tilde{\varepsilon}^\text{t}_{ij}D^\text{t}_{ijkl}\bigr) = \frac{\partial\tilde{\varepsilon}^\text{t}_{kl}}{\partial\tilde{\varepsilon}_{rs}}, \quad
        \frac{\partial}{\partial\tilde{\varepsilon}_{rs}}\bigl(\tilde{\varepsilon}^\text{c}_{ij}D^\text{t}_{ijkl}\bigr) = \frac{\partial\tilde{\varepsilon}^\text{c}_{kl}}{\partial\tilde{\varepsilon}_{rs}}.
    \end{aligned}
\end{equation*}
\end{remark}
\subsection{Type of anisotropy / material symmetry}\label{Sec:problem-anisotropy}
The presented method is general enough to apply for an arbitrary type of anisotropic elasticity tensors. Here we present three types of anisotropy, (a) cubic symmetry, (b) orthotropy and (c) full anisotropy, in Kelvin-matrix notation ($\undertilde{\bm{C}}$). 
Note that the components of $\undertilde{\bm{C}}$ are obtained assuming the orthonormal basis vectors are orientated along the material principal axes. Otherwise, a rotation of $\undertilde{\bm{C}}$ is required, see Remark \ref{Re:rotation}.
\paragraph{Cubic symmetry}
\begin{equation*}
    \begin{aligned}
        \undertilde{\bm{C}} = 
        \begin{bmatrix}
            \mathbb{C}_{1111} & \mathbb{C}_{1122} & \mathbb{C}_{1133} & 0 & 0 & 0 \\
            & \mathbb{C}_{1111} & \mathbb{C}_{2233} & 0 & 0 & 0 \\
            &  & \mathbb{C}_{1111} & 0 & 0 & 0 \\               &  &  & {2}\mathbb{C}_{2323} & 0 & 0 \\
            &  &  &  & {2}\mathbb{C}_{1313} & 0 \\
            &  &  &  &  & {2}\mathbb{C}_{1212}
        \end{bmatrix}
    \end{aligned}
\end{equation*}
\paragraph{Orthotropy}
    \begin{equation*}
        \begin{aligned}
            \undertilde{\bm{C}} = 
            \begin{bmatrix}
                \mathbb{C}_{1111} & \mathbb{C}_{1122} & \mathbb{C}_{1133} & 0 & 0 & 0 \\
                 & \mathbb{C}_{2222} & \mathbb{C}_{2233} & 0 & 0 & 0 \\
                 &  & \mathbb{C}_{3333} & 0 & 0 & 0 \\
                 &  &  & {2}\mathbb{C}_{2323} & 0 & 0 \\
                 &  &  &  & {2}\mathbb{C}_{1313} & 0 \\
                 &  &  &  &  & {2}\mathbb{C}_{1212}
            \end{bmatrix}
        \end{aligned}
    \end{equation*}
\paragraph{Full anisotropy}
\begin{equation*}
    \begin{aligned}
        \undertilde{\bm{C}} = 
        \begin{bmatrix}
            \mathbb{C}_{1111} & \mathbb{C}_{1122} & \mathbb{C}_{1133} & \sqrt{2}\mathbb{C}_{1123} & \sqrt{2}\mathbb{C}_{1113} & \sqrt{2}\mathbb{C}_{1112} \\
             & \mathbb{C}_{2222} & \mathbb{C}_{2233} & \sqrt{2}\mathbb{C}_{2223} & \sqrt{2}\mathbb{C}_{2213} & \sqrt{2}\mathbb{C}_{2212} \\
             &  & \mathbb{C}_{3333} & \sqrt{2}\mathbb{C}_{3323} & \sqrt{2}\mathbb{C}_{3313} & \sqrt{2}\mathbb{C}_{3312} \\
             &  &  & {2}\mathbb{C}_{2323} & 2\mathbb{C}_{2313} & 2\mathbb{C}_{2312} \\
             &  &  &  & {2}\mathbb{C}_{1313} & 2\mathbb{C}_{1312} \\
             &  &  &  &  & {2}\mathbb{C}_{1212}
        \end{bmatrix}
    \end{aligned}
\end{equation*}
\begin{remark}\label{Re:rotation}
We summarize how to transform $\undertilde{\bm{C}}$ to a coordinate system that does not coincide with the material principal axes. 
Below, $\undertilde{\mathbf{C}}^{\prime}$ is obtained via a transformation to a new basis ($x^\prime, y^\prime, z^\prime$):
\begin{equation}\label{Eq:rotation-p}
    \begin{aligned}
        \undertilde{\mathbf{C}}^{\prime} = \mathbf{P}\undertilde{\mathbf{C}}\mathbf{P}^\text{T},
    \end{aligned}
\end{equation}
where $\mathbf{P}$ denotes the transformation matrix.
In a special case, when the rotation is around the $z$-axis by an angle $\alpha$, $\mathbf{P}$ reduces to:
\begin{equation*}
    \begin{aligned}
        \mathbf{P} =
        \begin{bmatrix}
            c^2 & s^2 & 0 & 0 & 0 & \sqrt{2}cs \\
            s^2 & c^2 & 0 & 0 & 0 & -\sqrt{2}cs \\
            0 & 0 & 1 & 0 & 0 & 0 \\
            0 & 0 & 0 & c & -s & 0 \\
            0 & 0 & 0 & s & c & 0 \\
            -\sqrt{2}cs & \sqrt{2}cs & 0 & 0 & 0 & c^2-s^2 \\
        \end{bmatrix},
    \end{aligned}
\end{equation*}
where $c=\cos{\alpha}$, and $s=\sin{\alpha}$.
\end{remark}
% \subsection{Summary of the proposed model}\label{Sec:summary-model} {To account for the unilateral constraint due to the tension-compression asymmetry, two existing split models, namely VD and NT, are considered. For each model, \dots}
% \subsection{summary of equations}
% \paragraph{Volumetric-deviatoric split}
% Let $\undertilde{\mathbf{E}}_{3\times 3}$ be the $3\times 3$ matrix with all $1$'s and $\undertilde{\mathbf{I}}_{6\times 6}$ be the $6\times 6$ identity matrix. Then, the projection tensors ($\mathbb{D}^\text{t},~\mathbb{D}^\text{c}$) of \eqref{Eq:D_tensors} in matrix form read:
% \begin{subequations}\label{Eq:D_matrix}
%     \begin{align}
%         \undertilde{\mathbf{D}}^{t}
%         &= \frac13 H(\tr{\tilde{\bm{\varepsilon}}})
%         \begin{bmatrix}
%             \undertilde{\mathbf{E}}_{3\times 3} & \undertilde{\mathbf{0}}_{3\times 3} \\
%             \undertilde{\mathbf{0}}_{3\times 3} & \undertilde{\mathbf{0}}_{3\times 3} 
%         \end{bmatrix}
%         + \left(
%             \undertilde{\mathbf{I}}_{6\times 6} - \frac13     \begin{bmatrix}
%                 \undertilde{\mathbf{E}}_{3\times 3} & \undertilde{\mathbf{0}}_{3\times 3} \\
%             \undertilde{\mathbf{0}}_{3\times 3} & \undertilde{\mathbf{0}}_{3\times 3} 
%             \end{bmatrix}
%         \right), \\
%         \undertilde{\mathbf{D}}^{c} 
%         &= \frac13 H(-\tr{\tilde{\bm{\varepsilon}}})
%         \begin{bmatrix}
%             \undertilde{\mathbf{E}}_{3\times 3} & \undertilde{\mathbf{0}}_{3\times 3} \\
%             \undertilde{\mathbf{0}}_{3\times 3} & \undertilde{\mathbf{0}}_{3\times 3} 
%         \end{bmatrix}.
%     \end{align}
% \end{subequations}
% and
% \begin{subequations}\label{Eq:eps_matrix}
%     \begin{align}
%         \undertilde{\bm{\varepsilon}}^{t} = \Bigl(\undertilde{\mathbf{C}}^{\prime -1/2}\undertilde{\mathbf{D}}^{t}\undertilde{\mathbf{C}}^{\prime 1/2}\Bigr)\undertilde{\bm{\varepsilon}}, \\
%         \undertilde{\bm{\varepsilon}}^{c} = \Bigl(\undertilde{\mathbf{C}}^{\prime -1/2}\undertilde{\mathbf{D}}^{c}\undertilde{\mathbf{C}}^{\prime 1/2}\Bigr)\undertilde{\bm{\varepsilon}},
%     \end{align}
% \end{subequations}
% \begin{equation*}
%     \begin{aligned}
%         \varPsi^\text{t} = \frac12 g(d) (\undertilde{\bm{\varepsilon}}^\text{t})^\text{T}\undertilde{\bm{\varepsilon}}^\text{t}, \quad \varPsi^\text{c} = \frac12 (\undertilde{\bm{\varepsilon}}^\text{c})^\text{T}\undertilde{\bm{\varepsilon}}^\text{c}.
%     \end{aligned}
% \end{equation*}
% \begin{subequations}\label{Eq:C_matrix}
%     \begin{align}
%         \undertilde{\mathbf{C}}^{\prime t} &= \undertilde{\mathbf{C}}^{\prime -1}\undertilde{\mathbf{D}}^\text{t}\undertilde{\mathbf{C}}^{\prime}, \\
%         \undertilde{\mathbf{C}}^{\prime c} &= \undertilde{\mathbf{C}}^{\prime -1}\undertilde{\mathbf{D}}^\text{c}\undertilde{\mathbf{C}}^{\prime},
%     \end{align}
% \end{subequations}
% \begin{equation*}
%     \undertilde{\mathbf{C}}^{\prime} = g(d)\undertilde{\mathbf{C}}^{\prime t} + \undertilde{\mathbf{C}}^{\prime c}.
% \end{equation*}
% \begin{subequations}
%     \begin{align}
%         \undertilde{\bm{\sigma}}^{t}=\Bigl(\undertilde{\mathbf{C}^\prime}^{1/2}\mathbf{D}^{t}\undertilde{\mathbf{C}^\prime}^{1/2}\Bigr)\undertilde{\bm{\varepsilon}}, \\
%         \undertilde{\bm{\sigma}}^{c}=\Bigl(\undertilde{\mathbf{C}^\prime}^{1/2}\mathbf{D}^{c}\undertilde{\mathbf{C}^\prime}^{1/2}\Bigr)\undertilde{\bm{\varepsilon}},
%     \end{align}
% \end{subequations}
% \begin{equation*}
%     \begin{aligned}
%         \undertilde{\bm{\sigma}} = g(d)\undertilde{\bm{\sigma}}^\text{t} + \undertilde{\bm{\sigma}}^\text{c}.
%     \end{aligned}
% \end{equation*}

==> Crack Propagation in Orthotropic Materials/gtheta.tex <==
\section{Energy release rate computation: $G_\theta$ method}\label{App:G-theta}

The $G_{\theta}$ method is based on the estimation of the second derivatives of the energy potential with respect to crack length using the technique of virtual domain perturbation $\boldsymbol{\theta}$~\cite{Dubois1998}. 
Numerically it uses an integral over a surface, which is more accurate than the contour integral used in the J-integral~\cite{rice1968plane}. 
Denoting the tangential vector to the crack tip as $\bm{t}$, we can use the virtual domain perturbation:
\begin{equation}
 \boldsymbol{\theta} = f(r) \bm{t}
 ,
\end{equation}
where
\begin{equation}
f(r) = \begin{cases}
1 & \; \text{for } r < r_i \\
\dfrac{r-r_o}{r_i-r_o} & \; \text{for } r_i < r < r_o \\
0 & \; \text{for } r_o < r
\end{cases}
\end{equation}
and $r$ is the distance from the crack tip, and $r_i$ and $r_o$ are set as $r_i=4\ell$ and $r_o=2.5r_i$ in this study (Figure~\ref{fig:Gtheta_schematic}).
With $\boldsymbol{\theta}$, the energy release rate is computed as
\begin{equation}
\label{eq:gtheta}
G_\theta = \int_\Omega \boldsymbol{\sigma} : ( \nabla \mathbf{u} \nabla \boldsymbol{\theta} )
- \frac{1}{2} (\boldsymbol{\sigma}: \nabla \mathbf{u} ) \nabla \cdot \boldsymbol{\theta} \, \mathd x
.
\end{equation}

\begin{figure}[htbp]
\centering %
\subfigure[]{\includegraphics[width=0.35\linewidth]{Figs/shear_VolDev_0deg_tf_Gtheta.png}}
\quad
\subfigure[]{\includegraphics[width=0.25\linewidth]{Figs/magnify_shear_VolDev_0deg_tf_Gtheta.jpg}}\\
\subfigure{\includegraphics[width=0.3\linewidth]{Figs/Legend_shear_VolDev_0deg_tf_Gtheta.png}}

\caption{Phase field and $\theta$ profile  for \texttt{volumetric-deviatoric},  $\alpha=0$ at $t_f$ under shear loading.  We use virtual perturbation of $\theta$ to compute energy release rate using $G_{\theta}$. The  $\theta$ value is 1 inside of $B_{r_{i}}(P)$,  0 outside, and a linear interpolation in between. We set $r_{i}=4\ell$ and $r_{o}=2.5r_{i}$.}
\label{fig:Gtheta_schematic}
\end{figure}

However, the energy release rates computed by~\eqref{eq:gtheta} do not seem to predict the fracture propagation direction properly (Figure~\ref{fig:G_theta_sigma_plus} (a)). 
For this reason, considering the tension-compression asymmetry, we decompose $\mathbf{u}^t$ as
$$
\nabla \mathbf{u} = \nabla \mathbf{u}^t + \nabla \mathbf{u}^c
.
$$
Then we define the tensile part of the energy release rate as
\begin{equation}
\label{eq:gtheta_tens}
G_\theta^t = \int_\Omega \boldsymbol{\sigma}^t : ( \nabla \mathbf{u}^t \nabla \boldsymbol{\theta} )
- \frac{1}{2} (\boldsymbol{\sigma}^t: \nabla \mathbf{u}^t ) \nabla \cdot \boldsymbol{\theta} \, \mathd x
.
\end{equation}

While $\boldsymbol{\sigma}^t$ can be straightforwardly obtained from $\mathbb{C}\bm{\varepsilon}^t$, the tensile part of the displacement $\mathbf{u}^t$ is not defined in any of the strain energy split models.
Here, we assume that the compressive part of the displacement $\nabla \mathbf{u}^c$ is symmetric i.e., $(\nabla \mathbf{u}^c) = (\nabla \mathbf{u}^c)^\mathrm{T}$.
Then we have 
$$
\boldsymbol{\varepsilon}^c = \nabla \mathbf{u}^c
.
$$
and
\begin{equation}
\nabla \mathbf{u}^t 
= \nabla \mathbf{u} - \boldsymbol{\varepsilon}^c
.
\end{equation}
Figure~\ref{fig:G_theta_sigma_plus} illustrates the effects of the modified computation using the tensile part of the displacement, $G_\theta^t$ .
Without the modifications (Figure~\ref{fig:G_theta_sigma_plus} (a)), the maximum energy release rates point to an incorrect propagation direction (straight fracture propagation) prior to the propagation.
With our proposed modifications (Figure~\ref{fig:G_theta_sigma_plus} (b)), the direction predicted by the energy release rates coincide with the actual propagation direction.

\begin{figure}[htbp]
\centering %
\subfigure[ $G_{\theta}$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_shear_Masonry_0.png}}
\quad
\subfigure[$G_{\theta}^t$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_shear_Masonry_tensile_0.png}}
\caption{Comparison (a) energy release rate $G_{\theta}$ with (b) tensile part of energy release rate for \texttt{no-tension},  $\alpha=0$ under shear loading. In terms of directionality, tensile part of energy release rate accurately depicts the fracture propagation direction before and after fracture starts to propagate.}
\label{fig:G_theta_sigma_plus}
\end{figure}

==> Crack Propagation in Orthotropic Materials/introduction.tex <==
%Indicate the field of the work, why this field is important, and what has already been done (with proper citations).

%Indicate a gap, raise a research question, or challenge prior work in this territory. 

%Outline the purpose and announce the present research, clearly indicating what is novel and why it is significant.
%Avoid: repeating the abstract; providing unnecessary background information; exaggerating the importance of the work; claiming novelty without a proper literature search.
    The phase field method has steadily gained popularity for over a decade because of its convenience in simulating complex fracture processes, including crack nucleation, propagation, branching and merging~\cite{Bourdin2019}. The model was originally conceived as the variational formulation of brittle fracture by Francfort and Marigo~\cite{Francfort1998}, and its regularization by Bourdin et al~\cite{Bourdin2000}. The formulation solves crack problems by minimizing an energy functional that consists of the elastic energy and the crack surface energy. This significantly reduces the implementation complexities as the crack evolution is a natural outcome of the solution. Therefore, there is no need for a crack tracking algorithm or additional criteria for crack branching and merging. The method has found its extension in subjects such as composite failure~\cite{baldelli2014variational,Alessi2017, Yoshioka2021int}, ductility~\cite{alessi2014gradient, Ambati2015,Kuhn2016, miehe2016ductile,you2021brittle}, dynamic fracture~\cite{Bourdin2011, Borden2012,Nguyen2018, Yin2020}, hydraulic fracture~\cite{Bourdin2012, Wheeler2014, Wilson2016, Heider2017,zhou2018phase}, and environment assisted failure~\cite{martinez2018phase,schuler2020chemo} to name a few. \newline
    When mechanics of natural materials is concerned, especially geomaterials, they often exhibit anisotropic behaviors~\cite{carcione1995constitutive, Amadei1996,parisio2018formulation}.
    Anisotropic material response manifests itself in terms of deformation~\cite{nixon2010anisotropic, heng2015experimental} and/or preferential fracture propagation~\cite{wang2019anisotropic,li2021research}.
    In modeling anisotropy within the phase field framework, anisotropic fracture toughness has been mostly achieved through manipulation of the fracture surface energy term where one applies structural tensors~\cite{li2015phase,teichtmeister2017phase,bleyer2018phase,Li2019aniso,bilgen2021phase,gerasimov2022second} or assign direction dependent fracture toughness~\cite{bryant2018mixed,noii2020adaptive,fei2021double,rezaei2022anisotropic,gerasimov2022second,ulloa2022micromechanics} to encourage fracture propagation in certain directions. 
    While many studies are available for anisotropic fracture toughness, only a few have studied anisotropic constitutive model in phase field approaches~\cite{Nguyen2020, DIJK2020, luo2022phase}. \newline
    %In general, the solid endures partial loss of stiffness due to crack formation. To model this effect, the strain energy density and thus the stress tensor are degraded with respect to the evolution of the phase field. 
    Another material response to consider is tension-compression asymmetry in failure, i.e., a crack is less likely to propagate under compressive loadings. Consequently, there has to be a unilateral constraint in material degradation. Otherwise, unphysical crack propagation is predicted under compressive loading. How to account for this unilateral constraint is one of the main challenges in phase field modeling. 
    Note that such a model is sometimes referred to in the literature as an `anisotropic' phase field model \cite{Ambati2015}, however, in this work we use the term of `tension-compression asymmetry' for this effect (see also \cite{Moerman2016}), and preserve `anisotropy' to only address a material whose constitutive behavior is, unlike isotropic materials, directionally dependent. \newline
    With the need of tension-compression asymmetry in material degradation, several existing approaches consist of additively partitioning the sound elastic energy density $\varPsi$ into two portions, a crack-driving portion $\varPsi^\text{t}$ and a persistent portion $\varPsi^\text{c}$~\cite{Amor2009,Miehe2010_variational, Freddi2010,Steinke2018,wu2018length,de2021nucleation}.
    If we are able to partition the strain energy density based on the additive decomposition of the strain tensor, that is, 
    \begin{equation*}
        \begin{aligned}
            \bm{\varepsilon} = \bm{\varepsilon}^\text{t} + \bm{\varepsilon}^\text{c}, \quad \varPsi(\bm{\varepsilon}) = \varPsi^\text{t}(\bm{\varepsilon}^\text{t}) + \varPsi^\text{c}(\bm{\varepsilon}^\text{c}), \\
            \varPsi^\text{t}(\bm{\varepsilon}^\text{t}) = \frac12 \mathbb{C} \bm{\varepsilon}^\text{t}\cdot\bm{\varepsilon}^\text{t}, \quad %\bm{\sigma}^\text{t} = \mathbb{C}\bm{\varepsilon}^\text{t},\quad
            \varPsi^\text{c}(\bm{\varepsilon}^\text{t}) = \frac12 \mathbb{C} \bm{\varepsilon}^\text{c}\cdot\bm{\varepsilon}^\text{c}, %\bm{\sigma}^\text{c} = \mathbb{C}\bm{\varepsilon}^\text{c},
        \end{aligned}
    \end{equation*}
    the constitutive behaviors are characterized by the same elasticity tensor $\mathbb{C}$ where a dot $\cdot$ denotes the inner products between the two vectors or tensors of the same order. Then, there exists a local \emph{variational} principle from which several existing models can be derived:
    \begin{equation}\label{Eq:variational_principle}
        \begin{aligned}
            \bm{\varepsilon}^\text{t} = \underset{\bm{e}^\text{t}\in\mathcal{S}^\text{t}}{\mrm{argmin}} \, 
            \mathbb{C}\bigl(\bm{\varepsilon} - \bm{e}^\text{t}\bigr)\cdot\bigl(\bm{\varepsilon} - \bm{e}^\text{t}\bigr),
        \end{aligned}
    \end{equation}
    where the strain that contributes to damage ($\bm{\varepsilon}^\text{t}$) is defined as the orthogonal projection of the strain tensor $\bm{\varepsilon}$ onto the convex space $\mathcal{S}^\text{t}$ with respect to the energy norm defined by $\mathbb{C}$. Therefore, the modeling of tension-compression asymmetry in fracture response is reduced to the identification of such convex cone $\mathcal{S}^\text{t}$ to represent $\bm{\varepsilon}^\text{t}$~\cite{Freddi2010}. Also, $\bm{\varepsilon}^\text{c}$ is in a polar cone $\mathcal{S}^\text{c}=\Big\{\bm{e}^\text{c}\Big|\bm{e}^\text{c}\cdot\bm{e}^\text{t}\leq 0,~\forall\bm{e}^\text{t} \in \mathcal{S}^\text{t}\Big\}$. This way, we keep the variational structure of the crack problem by following the energy minimization. This is important because otherwise, one needs to introduce {ad hoc} criteria for the phase field problem. For more detailed analysis, we refer the readers to \cite{Marigo2016} and \cite{Freddi2010}. \newline
    % \subsection*{Challenge in materials with anisotropic nature}
    \emph{A challenges in anisotropic materials} is to satisfy this variational structure.
    From convex analysis, $\bm{\varepsilon}^\text{t}$ can be equivalently characterized by
    \begin{equation*}
        \begin{aligned}
            -\mathbb{C}(\bm{\varepsilon} - \bm{\varepsilon}^\text{t})\cdot\bigl(\bm{e}^\text{t} - \bm{\varepsilon}^\text{t}\bigr) \geq 0,
            \quad \forall \bm{e}^\text{t}\in\mathcal{S}^\text{t}.
        \end{aligned}
    \end{equation*}
    Testing this with $\bm{e}^\text{t}=2\bm{\varepsilon}^\text{t}$ and $\bm{e}^\text{t}=\frac{1}{2} \bm{\varepsilon}^\text{t}$ yields the following orthogonality condition~\cite{Li2016grad}:
    \begin{equation}\label{Eq:orthogonality}
        \begin{aligned}
            \mathbb{C}\bm{\varepsilon}^\text{t}\cdot\bm{\varepsilon}^\text{c} = \mathbb{C}\bm{\varepsilon}^\text{c}\cdot\bm{\varepsilon}^\text{t} = 0,
        \end{aligned}
    \end{equation}
    which is the necessary and sufficient condition for the strain energy density to be decomposed based on the partition of the strain tensor. However, for anisotropic linear elastic materials the principal directions of the stress and strain no longer coincide, i.e., the orthogonality condition is not generally satisfied:
    \begin{equation*}
        \begin{aligned}
            \mathbb{C}\bm{\varepsilon}^\text{t}\cdot\bm{\varepsilon}^\text{c} \neq 0 \text{~or~} \mathbb{C}\bm{\varepsilon}^\text{c}\cdot\bm{\varepsilon}^\text{t} \neq 0.
        \end{aligned}
    \end{equation*}
    {Therefore, further treatments are required in strain decomposition that keep the orthogonality condition for anisotropic materials.} \newline
    Recently, He and Shao \cite{He-2019} proposed an elastic energy preserving transformation so that an orthogonal decomposition of the strain tensor can be achieved in the transformed space. Therein, a rigorously orthogonal spectral decomposition of the strain tensor is performed.
    Thus, with the orthogonality condition being satisfied in the new space, the strain energy density of an anisotropic material is respectively partitioned into a crack-driving portion and a persistent portion. Moreover, to decompose the strain tensor in a two-dimensional setting, a set of closed-form coordinate-free expressions are provided.
    Nguyen et al. \cite{Nguyen2020} directly employed these expressions of strain decomposition into the phase field formulation, and compared the results with volumetric-deviatoric and spectral-decomposition for isotropic materials.
    % We notice a few other works also concerned with the decomposition of strain energy density of materials with anisotropic nature. 
    Van Dijk et al. \cite{DIJK2020} proposed a generalization of {volumetric-deviatoric} and spectral-decomposition to account for anisotropy of materials. Therein, the strain energy density is described as an isotropic tensor function of a type of tensorial square roots of the strain energy density.%\KYtodo{''some new types" may not be a good description}%
    \newline
    In this work, we present generalized formulations of two existing models for tension-compression asymmetry, a model by Amor et al. \cite{Amor2009} (henceforth referred to as {volumetric-deviatoric}) and a model by Freddi and Royer \cite{Freddi2010} (henceforth referred to as {no-tension}), to account for materials with anisotropic constitutive behavior in a three-dimensional setting. We borrow the basic concepts from \cite{He-2019} and perform the energy preserving transformation so that the orthogonality condition is preserved for a decomposition of an arbitrary anisotropic constitutive model. Then, we present the implementation details of {volumetric-deviatoric} and {no-tension} accounting for the anisotropy in Section \ref{Sec:problem-statement}. In addition, we provide a set of numerical examples to illustrate the capabilities of the present method in Section \ref{Sec:numerical-examples}. The results provide a step forward when developing phase field fracture theories for brittle materials with an anisotropic nature and highlight the importance of a proper decomposition of the strain energy density. \newline
    % {This paper proceeds as follows. In section \ref{Sec:problem-PF}, we recapitulate the basic ingredients of phase field formulation. Then, we proceed with an elastic energy preserving transformation so that an orthogonal decomposition of the strain tensor, and a partitioning of the strain energy density in a new space, is feasible. In section \ref{Sec:problem-unilateral}, we adopt two existing tension-compression asymmetry to \dots adjust the projection tensors and so on based on the two chosen models, the \texttt{volumetric-deviatoric} and \texttt{no-tension} models. In Section 3, two sets of numerical examples are provided. The effectiveness of model is shown, and the effect of orthotropy is realized and so on! Then, in Section \ref{Sec:numerical-examples} \dots}

==> Crack Propagation in Orthotropic Materials/mycommand.tex <==
\newcommand{\sigmaeff}{\sigma^{\mathit{eff}}}
\newcommand{\sigmavol}{\sigma_{\mathit{vol}}}
\newcommand{\ATone}{\texttt{AT$_1$}}
\newcommand{\ATtwo}{\texttt{AT$_2$}}
\newcommand{\KKL}{\texttt{KKL}}
\newcommand{\mrm}{\mathrm}
\newcommand{\Gc}{G_\mrm{c}}
\newcommand{\Gcomp}{\tilde{G}_\mrm{c}^{\mrm{int}} }
\newcommand{\Gbulk}{G_\mrm{c}^{\mrm{bulk}} }
\newcommand{\Gint}{G_\mrm{c}^{\mrm{int}} } 
\newcommand{\I}{\mathrm{I}}
\newcommand{\trp}{^{\scriptsize \text{T}}}
\newcommand{\itp}{^{\scriptsize -\text{T}}}
\newcommand{\sqrtp}{^{\scriptsize \text{T/2}}}
\newcommand{\isqrtp}{^{\scriptsize -\text{T/2}}}
\newcommand{\inv}{^{\scriptsize -1}}
\newcommand{\sqr}{^{\scriptsize \text{1/2}}}
\newcommand{\invsqr}{^{\scriptsize -\text{1/2}}}
\newcommand{\Haus}{\mathcal{H}^{N-1}}
\newcommand{\eps}{\varepsilon}
\newcommand{\Mac}[1]{\langle #1 \rangle}
\newcommand\ddfrac[2]{\frac{\displaystyle #1}{\displaystyle #2}}
\newcommand{\dcdot}{\boldsymbol :}
\newcommand{\mathd}{\mathrm{d}}
\newcommand{\mbf}[1]{{\mathbf{#1}}}
\newcommand{\jump}[1]{[\![#1]\!]}
\newcommand{\mbfs}{\boldsymbol}
% \newcommand{\Tr}[1]{\text{Tr} \left( #1\right) }
\newcommand\at[2]{\left.#1\right|_{#2}}
\newcommand{\normal}{\vec{n}_\Gamma}
\newcommand{\tileps}{\tilde{\bm{\varepsilon}}}

\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

\DeclareMathOperator{\e}{{\rm e}}
\DeclareMathOperator*{\argmin}{argmin}
\DeclareMathOperator{\tr}{tr}
\DeclareMathOperator{\dev}{dev}
\DeclareMathOperator{\divergence}{div}

\algtext*{EndIf}% Remove "end if" text
\algtext*{EndWhile}% Remove "end if" text
\algtext*{EndFor}% Remove "end if" text
\newtheorem{algo}{Algorithm}
\newtheorem{remark}{Remark}

\newcommand{\KYtodo}[1]{\todo[color=blue!40]{KY: #1}}
\newcommand{\KYtodoi}[1]{\todo[color=blue!40,inline]{KY: #1}}
\newcommand{\TNtodo}[1]{\todo[color=green!40]{TN: #1}}
\newcommand{\TNtodoi}[1]{\todo[color=green!40,inline]{TN: #1}}
\newcommand{\VZRtodo}[1]{\todo[color=red!40]{VZR: #1}}
\newcommand{\VZRtodoi}[1]{\todo[color=red!40,inline]{VZR: #1}}
\newcommand{\MMtodoi}[1]{\todo[color=orange!40,inline]{MM: #1}}

\definechangesauthor[name=VZR,color=brown]{VZR}

% \pdfstringdefDisableCommands{%
%   \def\\{}%
%   \def\texttt#1{<#1>}%
% }

==> Crack Propagation in Orthotropic Materials/mypackages.tex <==

\usepackage{amsmath,amsthm,amssymb,latexsym,amscd}
% \usepackage[shadow,textsize=small,textwidth=2.5cm]{todonotes}
\usepackage{geometry}
\usepackage{algorithm}
\usepackage{algpseudocode}
\usepackage{dsfont}
\usepackage{color}
\usepackage{lineno}
\usepackage{changes}
\usepackage[titletoc]{appendix}
\usepackage{url}
\usepackage{amsmath}
\usepackage{bm}
\usepackage{textgreek}
\usepackage{accents}
\usepackage{multirow}
\usepackage{subfigure}
\usepackage{caption}
\usepackage[bb=boondox]{mathalfa}
\usepackage{hyperref}

==> Crack Propagation in Orthotropic Materials/numerical_examples.tex <==
% \TNtodoi{Addition to the plots: add stress and strain ellipsoids (or rather the crosses of the principal axes scaled by principal values) to observe degree of anisotropy in stress and strain and (lack of) coaxiality quickly. Can be done with glyph plots in paraview which outputs principal stresses and directions. Yet to be implemented for strain, afaik.}
In order to verify our model, here we present two sets of numerical examples, a single edge notched tensile test and a shear test\footnote{The present model is implemented in the phase field process of an open source code, OpenGeoSys~\cite{Yoshioka2019}. Further information on the code and simulation examples are freely accessible at \url{https://www.opengeosys.org/} and~\cite{Bilke2019337}.}. 
The geometry and boundary conditions for both examples are shown in Figure \ref{Fig:geom_tensile} and \ref{Fig:geom_shear}, respectively. \newline
We consider a square plate ($0.001\,\text{m} \times 0.001\, \text{m}$) with an initial horizontal crack placed at the middle height from the left outer surface to the center of the specimen. The specimen was discretized by an unstructured mesh with approximately 41K and 64K standard {triangular} elements, respectively, for the tensile and shear tests. For each discretization, the mesh size of $h=4\times 10^{-6}$ m was used for the critical region of the expected crack path. The length scale parameter was chosen as {$\ell = 8\times 10^{-6}$} m which is small enough with respect to the specimen dimensions. Plane strain condition was assumed. Finally, the \ATtwo{} model was used in all simulations. \newline
The boundary conditions are as follows. The displacement along any direction on the bottom edge ($y=-L/2$) was fixed to zero. 
Also, the displacement at the top edge ($y = L/2$) was prescribed along the $y$-direction for the tensile test and the $x$-direction for the shear test, where the other direction was taken to be zero for both loading setup. 
The computation was performed with a monotonic displacement controlled loading with a constant displacement increment $\Delta\bm{u} = 2\times 10^{-7}$ m until $\Bar{\bm{u}} = 2 \times 10^{-6}$ m. Thereafter, the increment was adjusted to $\Delta\bm{u} = 1 \times 10^{-8}$ m until the last step at $\Bar{\bm{u}} = 2 \times 10^{-5}$ m. Also, the parameters used for an orthotropic material are listed in Table \ref{Tabs:material_properties}. Note that in both examples the critical surface energy $G_c$ was taken to be independent of the material orientation.
% the phase field $d > 0.6$ in one FE node.
\begin{table}[ht]
    \centering
    \begin{tabular}{c c c c}
    \hline
        Material Properties & Value & Unit \\ \hline
        $\nu_{23},\nu_{13},\nu_{12}$ & 0.17, 0.3, 0.52 & - \\ \hline
        $E_1,E_2,E_3$ & 210, 70, 210 & GPa \\ \hline
        $G_{23}, G_{13}, G_{12}$ & 46.63, 80.77, 46.63 & GPa \\ \hline
        $G_c$ & 2700 & N/m \\ \hline
\end{tabular}
    \caption{Orthotropic material properties used in this study, which were taken from van Dijk et al \cite{DIJK2020}.}
    \label{Tabs:material_properties}
\end{table}
\begin{figure}[htbp]
	\centering
	\subfigure[tensile test]{
		\begin{minipage}{0.45\linewidth}
			\centering
			\includegraphics[width=2.5in]{Figs/tension_schematic.png}
		\end{minipage}\label{Fig:geom_tensile}
	}
	\subfigure[shear test]{
		\begin{minipage}{0.45\linewidth}
			\centering
			\includegraphics[width=2.5in]{Figs/shear_schematic.png}
		\end{minipage}\label{Fig:geom_shear}
	}
	\caption{Schematic of two cracked square plate under a displacement (a) tensile and (b) shear loading. An  incremental displacement loading is applied on the top edges. The material principal axes ($\bm{e}_1,\bm{e}_2$) have an angle of $\alpha$ with the original coordinate system ($\bm{x},\bm{y}$).}
	\label{Fig:Configuration}
\end{figure}
\subsection{Tensile test}
A pre-notched square plate loaded in tension was computed. For orthotropic {volumetric-deviatoric} and {no-tension}, the fracture response at the last step $\Bar{\bm{u}}=2\times 10^{-5}$\,m is shown in Figure \ref{fig:tension-pf} with four material orientation angles $\alpha=0$, $\pm\pi/4$, and $\pi/2$. It was observed that both models generate similar crack paths. When the material principal axes coincide with the symmetric axes ($\alpha=0$ or $\alpha=\pi/2$), the crack moves straightforward. In other cases  ($\alpha=\pm\pi/4$), the crack slightly deviates from the straight path impacted by the orthotropic deformation. \newline
\begin{figure}[htbp]
\centering %
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = -\pi/4$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_VolDev_tension_45degneg.jpg}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = -\pi/4$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_Masonry_tension_45degneg.jpg}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = 0$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_VolDev_tension_0deg.jpg}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = 0$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_Masonry_tension_0deg.jpg}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = \pi/4$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_VolDev_tension_45deg.jpg}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = \pi/4$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_Masonry_tension_45deg.jpg}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = \pi/2$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_VolDev_tension_90deg.jpg}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = \pi/2$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_Masonry_tension_90deg.jpg}}
\caption{Cracked square plate under tension. Phase field contours of orthotropic {volumetric-deviatoric} and {no-tension} at the last step with with $\Bar{\bm{u}} = 2\times 10^{-5}$ m. The same parameters were used for both models. Under tensile loading, we observe a similar crack response for both models. With four material orientation angles tested for both models, the crack propagates along the horizontal axis for $\alpha=0$ and $\alpha=\pi/2$. For $\alpha=\pm\pi/4$, the crack deviates slightly for both models as a consequence of orthotropy.}
% However, the load-deflection curve illustrates the maximum load is significantly higher and earlier reached at $\alpha=\pi/2$ compared to $\alpha=0$. This is expected due to the orthotropy. 
% Also observed from the load-deflection curves is a complete loss in the global stiffness for all cases as soon as the crack reaches to the remote edge.
\label{fig:tension-pf}
\end{figure}
Figure~\ref{fig:tension-eps-ovd} depicts the magnitude of the strain tensor at the stage of the crack initiation for orthotropic {volumetric-deviatoric} with four material orientation angles. With $\alpha=0$ or $\alpha=\pi/2$, the deformation is symmetry around the $x$-axis whereas a non-symmetric behavior can be seen for $\alpha=\pm\pi/4$ where the material principal axes deviate from the symmetric axes. \newline
\begin{figure}[htbp]
\centering %
% 0.365 0.4735 0.3645 0.3005
\subfigure[$\alpha = -\pi/4$, $\bm{u} \approx 0.37\Bar{\bm{u}}$]{\includegraphics[width=0.4\linewidth]{Figs/eps_45degneg_540t_VolDev_tension_2.jpg}}
\quad
\subfigure[$\alpha = 0$, $\bm{u} \approx 0.47\Bar{\bm{u}}$]{\includegraphics[width=0.4\linewidth]{Figs/eps_0deg_757t_VolDev_tension_2.jpg}}
\quad
\subfigure[$\alpha = \pi/4$, $\bm{u} \approx 0.36 \Bar{\bm{u}}$]{\includegraphics[width=0.4\linewidth]{Figs/eps_45deg_539t_VolDev_tension_2.jpg}}
\quad
\subfigure[$\alpha = \pi/2$, $\bm{u} \approx 0.30 \Bar{\bm{u}}$]{\includegraphics[width=0.4\linewidth]{Figs/eps_90deg_411t_VolDev_tension_2.jpg}}\\
\subfigure{\includegraphics[width=0.25\linewidth]{Figs/legend_eps_tension_VolDev_2}}
\caption{The magnitude of the strain tensor at the initiation of the crack for orthotropic {volumetric-deviatoric} with four material orientation angles. A symmetric behavior is observed for $\alpha=0$ and $\alpha=\pi/2$, while the magnitude is higher for $\alpha=0$ as the material has more stiffness along the horizontal axis. For $\alpha=\pm\pi/4$, asymmetry is observed where the magnitude is higher along the material principal axis with more stiffness.}
% Also observed is the crack initiation occurs almost simultaneously for $\alpha=\pm\pi/4$ in the opposite vertical directions, while for $\alpha=\pi/2$ the crack starts earlier compared to $\alpha=0$. This is expected due to the orthotropy as the material is stiffer along the $y$-direction for $\alpha=\pi/2$.
\label{fig:tension-eps-ovd}
\end{figure}
Figure \ref{fig:tension-gt-curve} shows the energy release rate computation using the $G_{\theta}$ method with our proposed modifications (see~\ref{App:G-theta})  for both models with four material orientation angles. Crack propagation should follow the direction of the maximum energy dissipation~\cite{Hakim2009,Chambolle2009kink}. And it is observed that for all cases the maximum energy release rate directions are approximately along the crack paths.
 Moreover, both split models have the identical crack propagation paths under the tensile loading because the strain energies are all tensile and crack-driving. Also observed is the crack propagates at the same loading with $\alpha=\pm\pi/4$, but earlier with $\alpha=\pi/2$ than $\alpha=0$. This is because different stiffness in the principal loading direction require different displacement loads to build up the necessary strain energy for propagating the crack. \newline
\begin{figure}[htbp]
\centering %
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = -\pi/4$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_tension1_VolDev_45neg.png}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = -\pi/4$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_tension1_Masonry_45neg.png}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = 0$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_tension1_VolDev_0.png}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = 0$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_tension1_Masonry_0.png}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = \pi/4$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_tension1_VolDev_45.png}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = \pi/4$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_tension1_Masonry_45.png}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = \pi/2$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_tension1_VolDev_90.png}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = \pi/2$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_tension1_Masonry_90.png}}
% to add a colorbar here
\caption{Under tensile loading for orthotropic {volumetric-deviatoric} and {no-tension}, we computed the energy release rate using the $G_{\theta}$ method with our proposed modifications. Several curves are plotted for a set of $\Bar{\bm{u}}$ where the red ones correspond with the stage of crack initiation. The peak of each curve approximately aligns with the direction of crack propagation, see Figure \ref{fig:tension-pf}. For $\alpha=0$ and $\alpha=\pi/2$, the peaks are along the horizontal line, whereas for $\alpha=\pm\pi/4$ the peaks deviate slightly from the $x$-axis. In both models, crack initiation occurs almost at the same loading for $\alpha=\pm\pi/4$ but in the opposite vertical directions, while the crack starts to propagate earlier for $\alpha=\pi/2$ compared to $\alpha=0$. This is expected due to the effect of orthotropy as the material is stiffer along the $y$-direction for $\alpha=\pi/2$.}
%\MMtodoi{Font size is increased}
%\KYtodoi{I'd suggest to increase the font even more. The left half of the circle has no information so we can cover it with the legend.}
\label{fig:tension-gt-curve}
\end{figure}
% \begin{figure}[htbp]
% \centering %
% \subfigure[\texttt{volumetric-deviatoric}, $\alpha = -\pi/4$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_data_tension_VolDev_t_45neg.png}}
% \quad
% \subfigure[\texttt{no-tension}, $\alpha = -\pi/4$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_data_tension_Masonry_t_45neg.png}}
% \vskip\baselineskip
% \subfigure[\texttt{volumetric-deviatoric}, $\alpha = 0$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_data_tension_VolDev_t_0.png}}
% \quad
% \subfigure[\texttt{no-tension}, $\alpha = 0$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_data_tension_Masonry_t_0.png}}
% \vskip\baselineskip
% \subfigure[\texttt{volumetric-deviatoric}, $\alpha = \pi/4$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_data_tension_VolDev_t_45.png}}
% \quad
% \subfigure[\texttt{no-tension}, $\alpha = \pi/4$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_data_tension_Masonry_t_45.png}}
% \vskip\baselineskip
% \subfigure[\texttt{volumetric-deviatoric}, $\alpha = \pi/2$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_data_tension_VolDev_t_90.png}}
% \quad
% \subfigure[\texttt{no-tension}, $\alpha = \pi/2$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_data_tension_Masonry_t_90.png}}
% % to add a colorbar here
% \caption{The energy release rate ($G_{\theta}$) vs. displacement $\Bar{\bm{u}}$ is plotted for orthotropic {volumetric-deviatoric} and {no-tension} with four material orientation angles under the tensile loading. The maximum energy release rate is computed relatively higher than the critical surface energy \dots The vertical parts in the graphs indicate the cracks grow in an unstable manner, i.e., the crack advances a relatively large distance within one displacement increment.}
% % We use virtual perturbation of $\theta$ to compute the energy release rate
% \label{fig:tension-gt}
% \end{figure}

\subsection{Shear test}
Figure \ref{fig:shear-pf} depicts the crack paths for orthotropic {volumetric-deviatoric} and {no-tension} under shear loading with four material orientation angles ($\alpha=-\pi/4$, 0, $\pi/4$, and $\pi/2$). In contrary to the tensile test, herein a significant difference in crack response is observed between the two models for all cases.
\begin{figure}[htbp]
\centering %
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = -\pi/4$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_VolDev_shear_45degneg.jpg}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = -\pi/4$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_Masonry_shear_45degneg.jpg}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = 0$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_VolDev_shear_0deg.jpg}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = 0$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_Masonry_shear_0deg.jpg}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = \pi/4$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_VolDev_shear_45deg.jpg}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = \pi/4$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_Masonry_shear_45deg.jpg}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = \pi/2$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_VolDev_shear_90deg.jpg}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = \pi/2$]{\includegraphics[width=0.25\linewidth]{Figs/pf_tf_Masonry_shear_90deg.jpg}}
\caption{Cracked square plate under shear. Phase field contours of orthotropic {volumetric-deviatoric} and {no-tension} at the last step with $\Bar{\bm{u}} = 2\times 10^{-5}$ m. The same parameters were used for both models. Here, we observe that the crack paths are different depending on the model and the material orientation. For $\alpha=0$ and $\alpha=\pi/4$, however, both models generate relatively similar crack responses. 
With $\alpha=\pi/4$ there exist straight cracks that grow towards the lower right corner, almost along the material principal axis with lower stiffness. Also, with $\alpha=\pi/4$ the crack propagates earlier than other cases because of the effect of orthotropy. In this case, the material has the least stiffness along the preferred direction of crack growth under shear loading.}
\label{fig:shear-pf}
\end{figure}
Figure \ref{fig:shear-gt-curve} plots the maximum energy release rate for both models with four material orientation angles. In most cases, the peaks are approximately along the crack propagation paths. Note, however, that the maximum energy release rate computed is higher than the critical value which may require further investigation.
\begin{figure}[htbp]
\centering %
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = -\pi/4$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_shear_VolDev_tensile_45neg.png}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = -\pi/4$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_shear_Masonry_tensile_45neg.png}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = 0$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_shear_VolDev_tensile_0.png}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = 0$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_shear_Masonry_tensile_0.png}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = \pi/4$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_shear_VolDev_tensile_45.png}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = \pi/4$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_shear_Masonry_tensile_45.png}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, $\alpha = \pi/2$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_shear_VolDev_tensile_90.png}}
\quad
\subfigure[\texttt{no-tension}, $\alpha = \pi/2$]{\includegraphics[width=0.35\linewidth]{Figs/G_theta_Gcmax_polar_data_shear_Masonry_tensile_90.png}}
% to add a colorbar here
\caption{Under shear loading for orthotropic {volumetric-deviatoric} and {no-tension}, we computed the energy release rate using the $G_{\theta}$ method with our proposed modifications. Several curves are plotted for a set of $\Bar{\bm{u}}$ where the red curves correspond with the onset of crack propagation, and the orange ones refer to a fixed step thereafter for all samples, $\Bar{\bm{u}}=1.6\times 10^{-5}$ m,  where the crack is propagating towards the bottom-right corner. Like the tensile example, for most cases, the maximum energy release rate of each case approximately aligns with the direction of crack propagation (Figure \ref{fig:shear-pf}). An exception is the case of $\alpha=-\pi/4$ for {volumetric-deviatoric} where the peak of the red curve deviates from the direction of crack propagation, whereas the orange curve fits better. Also observed is that crack initiation occurs earlier in {no-tension} for all cases.}
\label{fig:shear-gt-curve}
\end{figure}
Figures \ref{fig:load-disp} show the load-deflection curves for the tensile examples (a--b) and the shear examples (c--d). All tensile examples result in a global stiffness loss, as the crack propagates through the sample. For the shear examples, only in one case ({volumetric-deviatoric} with $\alpha=\pi/2$), the crack reaches to the edge. In other cases, as soon as the crack propagates, the load drops. However this drop is not high and is recovered shortly in some cases.)
\begin{figure}[htbp]
\centering %
\subfigure[\texttt{volumetric-deviatoric}, tension]{\includegraphics[width=0.35\linewidth]{Figs/Load_disp_tension_VolDev.png}}
\quad
\subfigure[\texttt{no-tension}, tension]{\includegraphics[width=0.35\linewidth]{Figs/Load_disp_tension_Masonry.png}}
\vskip\baselineskip
\subfigure[\texttt{volumetric-deviatoric}, shear]{\includegraphics[width=0.35\linewidth]{Figs/Load_disp_shear_VolDev.png}}
\quad
\subfigure[\texttt{no-tension}, shear]{\includegraphics[width=0.35\linewidth]{Figs/Load_disp_shear_Masonry.png}}
\caption{Load deflection curves for both models under (a)--(b) tensile and (c)--(d) shear loading. For (a)--(b) a sudden loss of the stiffness indicates that the crack grows in an unstable manner. These load-displacment results show that the crack propagates at the same loading for $\alpha=\pm\pi/4$. For $\alpha=\pi/2$ the crack propagates earlier compared to $\alpha=0$ because the crack propagation direction aligns with the weaker material direction. For (c), the global stiffness is ``lost" for the case of $\alpha=\pi/2$ in which the crack reaches to the edge. Also observed for all cases in (c)--(d) is that there is a drop in the load at the onset of crack propagation.}
\label{fig:load-disp}
\end{figure}



==> auxil.tex <==
\subsubsection{Tension-compression asymmetry}
%Let $\mathcal{K}$ be the set of all symmetrized second-order tensors, and let $\mathcal{K}^t\in\mathcal{K}$ be a convex subset and $\mathcal{K}^c$ be a polar cone such that $\mathcal{K}^c = \{\bm{e}^c \, \big| \, \bm{e}^c \cdot \bm{e}^t \le 0 \quad  \forall\bm{e}^c \in \mathcal{K}^c \}$.
To account for tension-compression asymmetry, several existing approaches split the sound elastic energy density $\varPsi(\bm{\varepsilon})$ into a crack-driving portion $\varPsi^t(\bm{\varepsilon})$ and a persistent portion $\varPsi^c(\bm{\varepsilon})$. The elastic energy density in \eqref{Eq:pi} is then replaced by the expression
\begin{equation}\label{Eq:psi_deg}
    \begin{aligned}
        \varPsi = g(d)\varPsi^t + \varPsi^c,
    \end{aligned}
\end{equation}
where the damage degradation function $g(d)$ acts only on the crack-driving portion $\varPsi^t$.
We let the partition of the sound elastic energy density be based on that of the strain tensor \[\bm{\varepsilon} = \bm{\varepsilon}^t + \bm{\varepsilon}^c,\] that is, the constitutive behaviors
\begin{equation}\label{Eq:psi_split}
    \begin{aligned}
        \varPsi^t(\bm{\varepsilon}^t) = \frac12 \mathbb{C} \bm{\varepsilon}^t\cdot\bm{\varepsilon}^t, \quad \bm{\sigma}^t = \mathbb{C}\bm{\varepsilon}^t,\\
        \varPsi^c(\bm{\varepsilon}^t) = \frac12 \mathbb{C} \bm{\varepsilon}^c\cdot\bm{\varepsilon}^c, \quad \bm{\sigma}^c = \mathbb{C}\bm{\varepsilon}^c,
    \end{aligned}
\end{equation}
are characterized by the same elasticity tensor $\mathbb{C}$.
% An essential ingredient for developing phase field models resides in the additive decomposition of the strain tensor $\boldsymbol{\varepsilon}$ into a crack-driving portion $\bm{\varepsilon}^t$ and a persistent portion $\bm{\varepsilon}^{c}$ as below,
% \begin{equation}\label{Eq:eps_split}
%     \begin{aligned}
%         \bm{\varepsilon}=\bm{\varepsilon}^{t} + \bm{\varepsilon}^{c}.
%     \end{aligned}
% \end{equation}
% Following \citep{Freddi2010, li2016numerical}, we let the partition of the strain energy density $\varPsi(\bm{\varepsilon})$ be based on that of the strain tensor as in \eqref{Eq:eps_split} such that
\KYtodoi{We should mention other split methods available and emphasize that not all of them meet the orthogonality condition and why it is important to honor the orthogonality condition.}
% \begin{equation}\label{Eq:strain_eng_decomp}
%     \begin{aligned}
%         \varPsi(\bm{\varepsilon}) = \varPsi^t(\bm{\varepsilon}^t) + \varPsi^c(\bm{\varepsilon}^c).
%     \end{aligned}
% \end{equation}
%{For $\bm{\varepsilon}^t\in\mathcal{S}^t$ to be variationally consistent, we have:}
This way, $\bm{\varepsilon}^{t}\in\mathcal{K}^t$ can be determined based on the following variational requirement \citep{Freddi2010, li2016numerical}:
\begin{equation}\label{Eq:loc_variational}
    \begin{aligned}
        \bm{\varepsilon}^t = \underset{\bm{e}^t\in\mathcal{K}^t}{\mrm{argmin}} \, 
        \mathbb{C}\bigl(\bm{\varepsilon} - \bm{e}^t\bigr)\cdot\bigl(\bm{\varepsilon} - \bm{e}^t\bigr),
    \end{aligned}
\end{equation}
where $\mathcal{K}^t$ is a convex subset of the symmetrized second-order tensor. 
From convex analysis, the following inequality should be satisfied:
% Letting $f(\bm{e}^t):= \mathbb{C}(\bm{\varepsilon} - \bm{e}^t)\cdot(\bm{\varepsilon} - \bm{e}^t)$, the following inequality should be satisfied:
\begin{equation}\label{Eq:eps_min}
    \begin{aligned}
        -\mathbb{C}(\bm{\varepsilon} - \bm{\varepsilon}^t)\cdot\bigl(\bm{e}^t - \bm{\varepsilon}^t\bigr) \geq 0,
        % f(\bm{\varepsilon}^t) 
        % &\leq
        % f(\bm{\varepsilon}^t) + \nabla f(\bm{\varepsilon}^t)\cdot(\bm{\varepsilon}^t - \bm{e}^t) 
        % \quad \forall \bm{e}^t\in\mathcal{S}^t.
        % \nabla f(\bm{\varepsilon}^t)\cdot\bigl(\bm{\varepsilon}^t - \bm{e}^t\bigr) \geq 0,
        \quad \forall \bm{e}^t\in\mathcal{K}^t.
    \end{aligned}
\end{equation}
% or equivalently,
% \begin{equation}\label{Eq:eps_min}
%     \begin{aligned}
%         % \mathbb{C}(\bm{\varepsilon} - \bm{\varepsilon}^t)\cdot(\boldsymbol{\eps} - \boldsymbol{\eps}_+) 
%         % &\le
%         %  \mathbb{C}\dcdot(\boldsymbol{\eps} - \boldsymbol{\eps}_+)\dcdot(\boldsymbol{\eps} - \boldsymbol{\eps}_+)
%         % + 2 \mathbb{C}\dcdot(\boldsymbol{\eps} - \boldsymbol{\eps}_+)\dcdot(\boldsymbol{\eps}_+ - \bf{e}_+)
%         \mathbb{C}(\bm{\varepsilon} - \bm{\varepsilon}^t)\cdot(\bm{\varepsilon}^t - \bm{e}^t)\geq 0,
%         \quad \forall \bm{e}^t\in\mathcal{S}^t.
%     \end{aligned}
% \end{equation}
% Thus we have:
% \begin{equation}\label{Eq:eps_inequality}
%     \begin{aligned}
%         0\le \mathbb{C}\dcdot(\boldsymbol{\eps} - \boldsymbol{\eps}_+)\dcdot(\boldsymbol{\eps}_+ - \bf{e}_+).
%     \end{aligned}
% \end{equation}
Testing \eqref{Eq:eps_min} with $\bm{e}^t=2\bm{\varepsilon}^t$ and $\bm{e}^t=\frac{1}{2} \bm{\varepsilon}^t$ yields 
% \[ 0 \leq \mathbb{C} (\bm{\varepsilon}^c\cdot\bm{\varepsilon}^t) \quad \text{and} \quad 0 \leq - \mathbb{C} 
%     (\bm{\varepsilon}^c\cdot\bm{\varepsilon}^t).\]
%\[ \mathbb{C} (\bm{\varepsilon} - \bm{\varepsilon}^t)\cdot\bm{\varepsilon}^t \geq 0 \quad \text{and} \quad - \mathbb{C}  
%(\bm{\varepsilon} - \bm{\varepsilon}^t)\cdot\bm{\varepsilon}^t \geq 0.\]%
the following orthogonality condition:
\begin{equation}\label{Eq:orthogonality}
    \begin{aligned}
        % \mathbb{C}\dcdot\boldsymbol{\varepsilon}_{-}\dcdot\boldsymbol{\eps}_{+}=\mathbb{C}\dcdot\boldsymbol{\varepsilon}_+\dcdot\boldsymbol{\varepsilon}_{-}=0,
        \mathbb{C}\bm{\varepsilon}^t\cdot\bm{\varepsilon}^c = 0.
    \end{aligned}
\end{equation}
% Therefore, the strain energy of a linearly elastic material without damage 
% \[\varPsi(\boldsymbol{\varepsilon}) = \frac12\boldsymbol{\varepsilon}\dcdot\mathbb{C}\dcdot\boldsymbol{\varepsilon}\] 
% is partitioned into two parts which depend on $\bm{\varepsilon}^{t}$ and $\bm{\varepsilon}^{c}$ respectively:
% \begin{equation}\label{Eq:psi_split}
%     \begin{aligned}
%         \varPsi(\boldsymbol{\varepsilon}) = \varPsi^{t}(\boldsymbol{\varepsilon}_+)+\varPsi^{c}(\boldsymbol{\varepsilon}_{-})=\frac12\boldsymbol{\varepsilon}_+\dcdot\mathbb{C}\dcdot\boldsymbol{\varepsilon}_+ + \frac12\boldsymbol{\varepsilon}_-\dcdot\mathbb{C}\dcdot\boldsymbol{\varepsilon}_-.
%     \end{aligned}
% \end{equation}
% Therefore, the necessary and sufficient condition for \eqref{Eq:psi_split} to hold is the orthogonality condition \eqref{Eq:orthogonality}.
This implies that $\varPsi^t$ and $\varPsi^c$ defined in \eqref{Eq:psi_split} constitute indeed a partition of $\varPsi$
\begin{equation*}\label{Eq:psi_halb}
    \begin{aligned}
        2\varPsi = \mathbb{C}\bm{\varepsilon}\cdot\bm{\varepsilon} = \bm{\sigma}^t\cdot\bm{\varepsilon}^t + \bm{\sigma}^c\cdot\bm{\varepsilon}^c,
    \end{aligned}
\end{equation*}
where the crossed terms disappear thanks to the orthogonality condition \eqref{Eq:orthogonality}. \newline
Using this variational formulation in \eqref{Eq:loc_variational}, the tension-compression asymmetry reduces to setting the convex cone $\mathcal{K}^t$ which represents the strain that contributes to damage. \newline
In the sequel, we name two alternatives that we use in this paper.
\paragraph{volumetric-deviatoric}
\paragraph{masonry-like model}
% With the assumption that only the part $\varPsi_{0}(\boldsymbol{\varepsilon}_+)$ contributes to damage, the bulk strain energy of the material with damage takes the form:
% \begin{equation*}
%     \begin{aligned}
%         \varPsi^{\prime}(\boldsymbol{\varepsilon}) = g(d)\varPsi^{t}(\boldsymbol{\varepsilon}_+) + \varPsi^{c}({\boldsymbol{\varepsilon}_-}).
%     \end{aligned}
% \end{equation*}
% \TNtodoi{The degradation function is used here. Later, we should clearly distinguish between $\varPsi$ and $\varPsi_0$ as well as $\boldsymbol\sigma$ and $\boldsymbol\sigma _0$, etc. in the following derivations.}
% \VZRtodoi{Now, I changed $\varPsi_0$ to $\varPsi$ and the degraded $\varPsi$ to $\varPsi^{\prime}$, also introduced $\varPsi^t$ and $\varPsi^c$. I think it's better we first present our split, and the degradation function appears at very end of the stage.}
% %Let $\boldsymbol{\sigma}$ denote the Cauchy stress tensor.
\subsection{General approach to orthogonal decomposition}
\subsubsection*{Governing equations}
We aim at finding $(\bm{\varepsilon}^{t},\bm{\varepsilon}^{c})$ and correspondingly $(\bm{\sigma}^{t}, \bm{\sigma}^{c})$ such that the following set of equations holds:
\begin{subequations}\label{Eq:governing}
    \begin{align}
        \bm{\varepsilon} = \bm{\varepsilon}^{t} + \bm{\varepsilon}^{c}&, \\
        \mathbb{C}\bigl(\bm{\varepsilon}^{t}\cdot\bm{\varepsilon}^{c}\bigr) = 0&, \\
        \bm{\sigma} = \bm{\sigma}^{t} + \bm{\sigma}^{c}&, \\
        \mathbb{S}\bigl(\bm{\sigma}^{t}\cdot\bm{\sigma}^{c}\bigr) = 0&,
        %\boldsymbol{\sigma}^{t}\cdot(\mathbb{C}^{-1}\bm{\sigma}_{-})=0,
    \end{align}
\end{subequations}
where $\mathbb{S}=\mathbb{C}^{-1}$ denotes the compliance tensor, and \[\bm{\sigma}=\mathbb{C}\bm{\varepsilon}.\]
This way, we can partition $\varPsi(\bm{\varepsilon})$ as in \eqref{Eq:psi_split}.
